Controlled-squeeze gate in superconducting quantum circuits

We present a method to prepare non-classical states of the electromagnetic field in a microwave resonator. It is based on a controlled gate that applies a squeezing operation on a SQUID-terminated resonator conditioned on the state of a dispersively coupled qubit. This controlled-squeeze gate, when combined with Gaussian operations on the resonator, is universal. We explore the use of this tool to map an arbitrary qubit state into a superposition of squeezed states. In particular, we target a bosonic code with well-defined superparity which makes photon losses detectable by non-demolition parity measurements. We analyze the possibility of implementing this using state-of-the-art circuit QED tools and conclude that it is within reach of current technologies.

==> bib.tex <==
@book{guckenheimer2013,
  title={Nonlinear oscillations, dynamical systems, and bifurcations of vector fields},
  author={Guckenheimer, John and Holmes, Philip},
  volume={42},
  year={2013},
  publisher={Springer Science \& Business Media}
}

@article{milisec,
author = {Suhas Ganjam and Yanhao Wang and Yao Lu and Archan Banerjee and Chan U Lei and Lev Krayzman and Kim Kisslinger and Chenyu Zhou and Ruoshui Li and Yichen Jia and Mingzhao Liu and Luigi Frunzio and Robert J. Schoelkopf },
title = {Surpassing millisecond coherence in on chip superconducting quantum memories by optimizing materials and circuit design},
journal = {Nature Communications},
volume = {15},
number = {3687},
pages = {},
year = {2024},
doi = {https://doi.org/10.1038/s41467-024-47857-6},
URL = {},
}

@article{reinhold,
author = {P. Reinhold},
title = {Controlling error-correctable bosonic qubits},
journal = {Ph.D.
thesis, Yale University},
volume = {},
number = {},
pages = {},
year = {2019},
doi = {},
URL = {},
}


@article{puri2020,
author = {Shruti Puri  and Lucas St-Jean  and Jonathan A. Gross  and Alexander Grimm  and Nicholas E. Frattini  and Pavithran S. Iyer  and Anirudh Krishna  and Steven Touzard  and Liang Jiang  and Alexandre Blais  and Steven T. Flammia  and S. M. Girvin },
title = {Bias-preserving gates with stabilized cat qubits},
journal = {Science Advances},
volume = {6},
number = {34},
pages = {eaay5901},
year = {2020},
doi = {10.1126/sciadv.aay5901},
URL = {https://www.science.org/doi/abs/10.1126/sciadv.aay5901},
}


@article{teoh2023dual,
  title={Dual-rail encoding with superconducting cavities},
  author={Teoh, James D and Winkel, Patrick and Babla, Harshvardhan K and Chapman, Benjamin J and Claes, Jahan and de Graaf, Stijn J and Garmon, John WO and Kalfus, William D and Lu, Yao and Maiti, Aniket and others},
  journal={Proceedings of the National Academy of Sciences},
  volume={120},
  number={41},
  pages={e2221736120},
  year={2023},
  publisher={National Acad Sciences}
}

@article{eickbush-thesis,
    author = {Alec Eickbusch},
    title = {Quantum Control and Error Correction of Grid States in a Superconducting Oscillator},
    journal = {Yale University, ProQuest Dissertations \& Theses, 30991810},
    year = {2024} 
}

@article{lombjpp,
    author = {Fernando C. Lombardo and Juan Pablo Paz},
    title = {Controlled-squeeze gate},
    journal = {in preparation},
    year = {2025}
}

@article{Fasel,
    author = {T. F\"osel and S. Krastanov and  F. Marquardt and L. Jiang },
    title = {Efficient cavity control with SNAP gates},
    journal = {arXiv:2004.14256},
    year = {2024}
}

@article{lambda4,
    author = {J R Johansson and G Johansson and C M Wilson and F Nori},
    title = {Dynamical Casimir effect in superconducting microwave circuits},
    journal = {Phys. Rev. A 82, 052509 },
    year = {2010}
}


@article{Squeezing-njp,
    author = {L Zhong and E P Menzel and R Di Candia and P Eder and M Ihmig and A Baust and M Haeberlein and E Hoffmann and K Inomata and T Yamamoto and Y Nakamura and E Solano and F Deppe and A Marx and R Gross},
    title = {Squeezing with a flux-driven Josephson parametric amplifier},
    journal = { New J. Phys. 15 125013},
    year = {2013}
}

@article{transmon-2007,
    author = {Jens Koch and Terri M. Yu and  Jay Gambetta and A. A. Houck and D. I. Schuster and J. Majer and  Alexandre Blais and  Michel H. Devoret and Steven M. Girvin and Robert J. Schoelkopf},
    title = {Charge-insensitive qubit design derived from the Cooper pair box},
    journal = {Physical Review A 76, 042319 },
    year = {2007}
}
@article{splitting,
    author = {D. I. Schuster and A. A. Houck and J. A. Schreier and A. Wallraff and J. M. Gambetta and A. Blais and L. Frunzio and J. Majer and B. Johnson and M. H. Devoret and S. M. Girvin and R. J. Schoelkopf},
    title = {Resolving photon number states in a superconducting circuit},
    journal = {Nature volume 445, pages515–518},
    year = {2007} 
}
@article{delsing-snail,
    author = {Yong Lu and Marina Kudra and  Timo Hillmann and
Jiaying Yang and Hang-Xi Li and Fernando Quijandría and Per Delsing},
    title = {Resolving Fock states near the Kerr-free point of a
superconducting resonator},
    journal = {npj Quantum Information 9:114},
    year = {2023}
}

@article{wineland-science,
    author = {Burd, S. C. and Srinivas, R. and Bollinger, R. R. and Wilson, A. C. and Wineland, D. J. and Leibfried, D. and Slichter, D. H. and Allcock, D. T. C.},
    title = {Quantum amplification of mechanical oscillator motion},
    journal = {Science 364, 1163-1165},
    year = {2019}
}

@article{wang,
    author = {W. Wang and et al },
    title = {Converting Quasiclassical States into Ar- bitrary Fock State Superpositions in a Superconducting Circuit},
    journal = {Physical Review Letters 118, 223604},
    year = {2017}
}

@article{khanje,
    author = {N. Khaneja and T. Reiss and  C. Kehlet and  T. Schulte-Herbr\"uggen and S.J. Glaser, S. J.},
    title = {Optimal control of coupled spin dy- namics: Design of NMR pulse sequences by gradient as- cent algorithms},
    journal = {Journal of Magnetic Resonance 172, 296–305},
    year = {2005}
}

@article{heers2,
    author = {R.W. Heeres and et al},
    title = {Implementing a universal gate set on a logical qubit encoded in an oscillator},
    journal = {Nature Communications 8, 94 },
    year = {2017}
}

@article{riehold,
    author = {P. Reinhold},
    title = {Controlling Error-Correctable Bosonic Qubits},
    journal = {Ph.D. thesis, Yale University},
    year = {2019}
}

@article{Ma,
    author = {W.-L. Ma and et al},
    title = {Quantum control of bosonic modes with superconducting circuits},
    journal = {Science Bulletin 66, 1789–1805},
    year = {2021}
}

@article{ni2023beating,
  title={Beating the break-even point with a discrete-variable-encoded logical qubit},
  author={Ni, Zhongchu and Li, Sai and Deng, Xiaowei and Cai, Yanyan and Zhang, Libo and Wang, Weiting and Yang, Zhen-Biao and Yu, Haifeng and Yan, Fei and Liu, Song and others},
  journal={Nature},
  volume={616},
  number={7955},
  pages={56--60},
  year={2023},
  publisher={Nature Publishing Group UK London}
}



@article{Grimsmo2020,
  title = {Quantum Computing with Rotation-Symmetric Bosonic Codes},
  author = {Grimsmo, Arne L. and Combes, Joshua and Baragiola, Ben Q.},
  journal = {Phys. Rev. X},
  volume = {10},
  issue = {1},
  pages = {011058},
  numpages = {32},
  year = {2020},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevX.10.011058},
  url = {https://link.aps.org/doi/10.1103/PhysRevX.10.011058}
}

@article{Paik2011,
  title = {Observation of High Coherence in Josephson Junction Qubits Measured in a Three-Dimensional Circuit QED Architecture},
  author = {Paik, Hanhee and Schuster, D. I. and Bishop, Lev S. and Kirchmair, G. and Catelani, G. and Sears, A. P. and Johnson, B. R. and Reagor, M. J. and Frunzio, L. and Glazman, L. I. and Girvin, S. M. and Devoret, M. H. and Schoelkopf, R. J.},
  journal = {Phys. Rev. Lett.},
  volume = {107},
  issue = {24},
  pages = {240501},
  numpages = {5},
  year = {2011},
  month = {Dec},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.107.240501},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.107.240501}
}


@article{wang2022towards,
  title={Towards practical quantum computers: Transmon qubit with a lifetime approaching 0.5 milliseconds},
  author={Wang, Chenlu and Li, Xuegang and Xu, Huikai and Li, Zhiyuan and Wang, Junhua and Yang, Zhen and Mi, Zhenyu and Liang, Xuehui and Su, Tang and Yang, Chuhong and others},
  journal={npj Quantum Information},
  volume={8},
  number={1},
  pages={3},
  year={2022},
  publisher={Nature Publishing Group UK London}
}


@article{andersen2024thermalization,
      title={Thermalization and Criticality on an Analog-Digital Quantum Simulator}, 
      author={Trond I. Andersen and Nikita Astrakhantsev and Amir Karamlou and Xiao Mi},
journal={Nature (London)},
  volume={638},
  number={},
  pages={79},      
year={2025},
}


@article{sivak2022, title={Real-time quantum error correction beyond break-even}, volume={616}, url={http://dx.doi.org/10.1038/s41586-023-05782-6}, DOI={10.1038/s41586-023-05782-6}, number={7955}, journal={Nature}, publisher={Springer Science and Business Media LLC}, author={Sivak, V. V. and Eickbusch, A. and Royer, B. and Singh, S. and Tsioutsios, I. and Ganjam, S. and Miano, A. and Brock, B. L. and Ding, A. Z. and Frunzio, L. and Girvin, S. M. and Schoelkopf, R. J. and Devoret, M. H.}, year={2023}, month=mar, pages={50–55}, language={en} }

@article{Gottesman2001,
  title = {Encoding a qubit in an oscillator},
  author = { Gottesman, Daniel and Kitaev, Alexei and Preskill, John},
  journal = {Phys. Rev. A},
  volume = {64},
  issue = {1},
  pages = {012310},
  numpages = {21},
  year = {2001},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.64.012310},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.64.012310}, mynote = {Theses states were introduced by Gotesman Kitaev preskill (GKP) in the seminal paper:}

}


@article{houck2012chip,
  title={On-chip quantum simulation with superconducting circuits},
  author={Houck, Andrew A and T{\"u}reci, Hakan E and Koch, Jens},
  journal={Nature Physics},
  volume={8},
  number={4},
  pages={292--299},
  year={2012},
  publisher={Nature Publishing Group UK London}
}

@article{reed2012realization,
  title={Realization of three-qubit quantum error correction with superconducting circuits},
  author={Reed, Matthew D and DiCarlo, Leonardo and Nigg, Simon E and Sun, Luyan and Frunzio, Luigi and Girvin, Steven M and Schoelkopf, Robert J},
  journal={Nature},
  volume={482},
  number={7385},
  pages={382--385},
  year={2012},
  publisher={Nature Publishing Group UK London}
}

@article{koch2007,
  title = {Charge-insensitive qubit design derived from the Cooper pair box},
  author = {Koch, Jens and Yu, Terri M. and Gambetta, Jay and Houck, A. A. and Schuster, D. I. and Majer, J. and Blais, Alexandre and Devoret, M. H. and Girvin, S. M. and Schoelkopf, R. J.},
  journal = {Phys. Rev. A},
  volume = {76},
  issue = {4},
  pages = {042319},
  numpages = {19},
  year = {2007},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.76.042319},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.76.042319}
}





@article{ganjam2024surpassing,
  title={Surpassing millisecond coherence in on chip superconducting quantum memories by optimizing materials and circuit design},
  author={Ganjam, Suhas and Wang, Yanhao and Lu, Yao and Banerjee, Archan and Lei, Chan U and Krayzman, Lev and Kisslinger, Kim and Zhou, Chenyu and Li, Ruoshui and Jia, Yichen and others},
  journal={Nature Communications},
  volume={15},
  number={1},
  pages={3687},
  year={2024},
  publisher={Nature Publishing Group UK London}
}

@article{khaneja2005optimal,
  title={Optimal control of coupled spin dynamics: design of NMR pulse sequences by gradient ascent algorithms},
  author={Khaneja, Navin and Reiss, Timo and Kehlet, Cindie and Schulte-Herbr{\"u}ggen, Thomas and Glaser, Steffen J},
  journal={Journal of magnetic resonance},
  volume={172},
  number={2},
  pages={296--305},
  year={2005},
  publisher={Elsevier}
}

@article{leghtas2013deterministic,
  title={Deterministic protocol for mapping a qubit to coherent state superpositions in a cavity},
  author={Leghtas, Zaki and Kirchmair, Gerhard and Vlastakis, Brian and Devoret, Michel H and Schoelkopf, Robert J and Mirrahimi, Mazyar},
  journal={Physical Review A},
  volume={87},
  number={4},
  pages={042315},
  year={2013},
  publisher={APS}
}


@article{heeres2017implementing,
  title={Implementing a universal gate set on a logical qubit encoded in an oscillator},
  author={Heeres, Reinier W and Reinhold, Philip and Ofek, Nissim and Frunzio, Luigi and Jiang, Liang and Devoret, Michel H and Schoelkopf, Robert J},
  journal={Nature communications},
  volume={8},
  number={1},
  pages={94},
  year={2017},
  publisher={Nature Publishing Group UK London}
}


@article{Krastanov2015,
  title = {Universal control of an oscillator with dispersive coupling to a qubit},
  author = {Krastanov, Stefan and Albert, Victor V. and Shen, Chao and Zou, Chang-Ling and Heeres, Reinier W. and Vlastakis, Brian and Schoelkopf, Robert J. and Jiang, Liang},
  journal = {Phys. Rev. A},
  volume = {92},
  issue = {4},
  pages = {040303},
  numpages = {5},
  year = {2015},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.92.040303},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.92.040303}
}


@article{Kundra2022,
  title = {Robust Preparation of Wigner-Negative States with Optimized SNAP-Displacement Sequences},
  author = {Kudra, Marina and Kervinen, Mikael and Strandberg, Ingrid and Ahmed, Shahnawaz and Scigliuzzo, Marco and Osman, Amr and Lozano, Daniel P\'erez and Thol\'en, Mats O. and Borgani, Riccardo and Haviland, David B. and Ferrini, Giulia and Bylander, Jonas and Kockum, Anton Frisk and Quijandr\'{\i}a, Fernando and Delsing, Per and Gasparinetti, Simone},
  journal = {PRX Quantum},
  volume = {3},
  issue = {3},
  pages = {030301},
  numpages = {12},
  year = {2022},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/PRXQuantum.3.030301},
  url = {https://link.aps.org/doi/10.1103/PRXQuantum.3.030301}
}


@article{storz2023loophole,
  title={Loophole-free Bell inequality violation with superconducting circuits},
  author={Storz, Simon and Sch{\"a}r, Josua and Kulikov, Anatoly and Magnard, Paul and Kurpiers, Philipp and L{\"u}tolf, Janis and Walter, Theo and Copetudo, Adrian and Reuer, Kevin and Akin, Abdulkadir and others},
  journal={Nature},
  volume={617},
  number={7960},
  pages={265--270},
  year={2023},
  publisher={Nature Publishing Group UK London}
}



@article{haroche2020cavity,
  title={From cavity to circuit quantum electrodynamics},
  author={Haroche, S and Brune, M and Raimond, JM},
  journal={Nature Physics},
  volume={16},
  number={3},
  pages={243--246},
  year={2020},
  publisher={Nature Publishing Group UK London}
}



@article{google2023suppressing,
  title={Suppressing quantum errors by scaling a surface code logical qubit},
  journal={Nature},
  volume={614},
  number={7949},
  pages={676--681},
  year={2023},
  publisher={Nature Publishing Group UK London}
}


@article{Devoret1985,
  title = {Measurements of Macroscopic Quantum Tunneling out of the Zero-Voltage State of a Current-Biased Josephson Junction},
  author = {Devoret, Michel H. and Martinis, John M. and Clarke, John},
  journal = {Phys. Rev. Lett.},
  volume = {55},
  issue = {18},
  pages = {1908--1911},
  numpages = {0},
  year = {1985},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.55.1908},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.55.1908}
}



@article{Heeres2016,
  title = {Cavity State Manipulation Using Photon-Number Selective Phase Gates},
  author = {Heeres, Reinier W. and Vlastakis, Brian and Holland, Eric and Krastanov, Stefan and Albert, Victor V. and Frunzio, Luigi and Jiang, Liang and Schoelkopf, Robert J.},
  journal = {Phys. Rev. Lett.},
  volume = {115},
  issue = {13},
  pages = {137002},
  numpages = {5},
  year = {2015},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.115.137002},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.115.137002}
}


@article{sayrin2011,
  title={Real-time quantum feedback prepares and stabilizes photon number states},
  author={Sayrin, Cl{\'e}ment and Dotsenko, Igor and Zhou, Xingxing and Peaudecerf, Bruno and Rybarczyk, Th{\'e}o and Gleyzes, S{\'e}bastien and Rouchon, Pierre and Mirrahimi, Mazyar and Amini, Hadis and Brune, Michel and others},
  journal={Nature},
  volume={477},
  number={7362},
  pages={73--77},
  year={2011},
  publisher={Nature Publishing Group UK London}
}

@article{teixeira2020,
  title={Preparation of long-lived, non-autoionizing circular Rydberg states of strontium},
  author={Teixeira, RC and Larrouy, A and Muni, A and Lachaud, L and Raimond, J-M and Gleyzes, S and Brune, M},
  journal={Physical Review Letters},
  volume={125},
  number={26},
  pages={263001},
  year={2020},
  publisher={APS}
}


@article{dietsche2019,
  title={High-sensitivity magnetometry with a single atom in a superposition of two circular Rydberg states},
  author={Dietsche, EK and Larrouy, A and Haroche, S and Raimond, JM and Brune, Michel and Gleyzes, S},
  journal={Nature Physics},
  volume={15},
  number={4},
  pages={326--329},
  year={2019},
  publisher={Nature Publishing Group UK London}
}

@misc{venkatraman2022,
  doi = {10.48550/ARXIV.2211.04605},
  
  url = {https://arxiv.org/abs/2211.04605},
  
  author = {Venkatraman, Jayameenakshi and Cortinas, Rodrigo G. and Frattini, Nicholas E. and Xiao, Xu and Devoret, Michel H.},
  
  keywords = {Quantum Physics (quant-ph), Mesoscale and Nanoscale Physics (cond-mat.mes-hall), Atomic Physics (physics.atom-ph), FOS: Physical sciences, FOS: Physical sciences},
  
  title = {Quantum interference of tunneling paths under a double-well barrier},
  
  publisher = {arXiv},
  
  year = {2022},
  
  copyright = {Creative Commons Attribution 4.0 International}
}


@article{Goto2021,
  title = {Chaos in coupled Kerr-nonlinear parametric oscillators},
  author = {Goto, Hayato and Kanao, Taro},
  journal = {Phys. Rev. Research},
  volume = {3},
  issue = {4},
  pages = {043196},
  numpages = {12},
  year = {2021},
  month = {Dec},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevResearch.3.043196},
  url = {https://link.aps.org/doi/10.1103/PhysRevResearch.3.043196}
}

@article{chono2022,
  title = {Two-qubit gate using conditional driving for highly detuned Kerr nonlinear parametric oscillators},
  author = {Chono, Hiroomi and Kanao, Taro and Goto, Hayato},
  journal = {Phys. Rev. Res.},
  volume = {4},
  issue = {4},
  pages = {043054},
  numpages = {8},
  year = {2022},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevResearch.4.043054},
  url = {https://link.aps.org/doi/10.1103/PhysRevResearch.4.043054}
}


@article{Hirschfelder1939,
author = {Hirschfelder,J. O.  and Wigner,E. },
title = {Some Quantum‐Mechanical Considerations in the Theory of Reactions Involving an Activation Energy},
journal = {The Journal of Chemical Physics},
volume = {7},
number = {8},
pages = {616-628},
year = {1939},
doi = {10.1063/1.1750500},
URL = { 
        https://doi.org/10.1063/1.1750500    
},
}

@article{larkin1984,
  title={Quantum-mechanical tunneling sith dissipation. The pre-exponential factor},
  author={Larkin, AI and Ovchinnikov, Yu N},
  journal={Zh. Eksp. Teor. Fiz},
  volume={86},
  pages={726},
  year={1984}
}

@Unpublished{ruiz2022,

  author = {Ruiz, Diego and Gautier, Ronan and Guillaud, Jérémie and Mirrahimi, Mazyar},

  
  title = {Two-photon driven Kerr quantum oscillator with multiple spectral degeneracies},
  year = {2022},
  eprint = {2211.03689},
  archivePrefix = "arXiv",
  primaryClass = "quant-ph",
}

@article{Oliva2019,
  title = {Quantum Kerr oscillators' evolution in phase space: Wigner current, symmetries, shear suppression, and special states},
  author = {Oliva, Maxime and Steuernagel, Ole},
  journal = {Phys. Rev. A},
  volume = {99},
  issue = {3},
  pages = {032104},
  numpages = {7},
  year = {2019},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.99.032104},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.99.032104}
}


@article{marthaler2006_,
  title = {Switching via quantum activation: A parametrically modulated oscillator},
  author = {Marthaler, M. and Dykman, M. I.},
  journal = {Phys. Rev. A},
  volume = {73},
  issue = {4},
  pages = {042108},
  numpages = {14},
  year = {2006},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.73.042108},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.73.042108}
}

@Unpublished{gravina2022,
  doi = {10.48550/ARXIV.2208.04928},
  url = {https://arxiv.org/abs/2208.04928},
  
  author = {Gravina, Luca and Minganti, Fabrizio and Savona, Vincenzo},
  
  title = {A critical Schrödinger cat qubit},
  
  year = {2022},
  eprint = {2208.04928},
  archivePrefix = "arXiv",
  primaryClass = "quant-ph",
}

@article{Hanggi1990,
  title = {Reaction-rate theory: fifty years after Kramers},
  author = {H\"anggi, Peter and Talkner, Peter and Borkovec, Michal},
  journal = {Rev. Mod. Phys.},
  volume = {62},
  issue = {2},
  pages = {251--341},
  numpages = {0},
  year = {1990},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/RevModPhys.62.251},
  url = {https://link.aps.org/doi/10.1103/RevModPhys.62.251}
}







@article{Weiner1978,
author = {Weiner,J. H. },
title = {Quantum rate theory for a symmetric double‐well potential},
journal = {The Journal of Chemical Physics},
volume = {68},
number = {5},
pages = {2492-2506},
year = {1978},
doi = {10.1063/1.435977},

URL = { 
        https://doi.org/10.1063/1.435977
    
},
eprint = { 
        https://doi.org/10.1063/1.435977
    
}

}



@Unpublished{chavez2022,
  doi = {10.48550/ARXIV.2210.07255},
  
  url = {https://arxiv.org/abs/2210.07255},
  
  author = {Chávez-Carlos, Jorge and Lezama, Talía L. M. and Cortiñas, Rodrigo G. and Venkatraman, Jayameenakshi and Devoret, Michel H. and Batista, Victor S. and Pérez-Bernal, Francisco and Santos, Lea F.},
  
  title = {Spectral kissing and its dynamical consequences in the squeezed Kerr-nonlinear oscillator},
  
  year = {2022},
  eprint = {2210.07255},
  archivePrefix = "arXiv",
  primaryClass = "quant-ph",
}


@article{dykman2011_,
  title = {Quantum heating of a parametrically modulated oscillator: Spectral signatures},
  author = {Dykman, M. I. and Marthaler, M. and Peano, V.},
  journal = {Phys. Rev. A},
  volume = {83},
  issue = {5},
  pages = {052115},
  numpages = {10},
  year = {2011},
  month = {May},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.83.052115},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.83.052115}
}

@article{Wigner1932,
  title = {On the Quantum Correction For Thermodynamic Equilibrium},
  author = {Wigner, E.},
  journal = {Phys. Rev.},
  volume = {40},
  issue = {5},
  pages = {749--759},
  numpages = {0},
  year = {1932},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRev.40.749},
  url = {https://link.aps.org/doi/10.1103/PhysRev.40.749}
}


@article{kramers1940,
  title={Brownian motion in a field of force and the diffusion model of chemical reactions},
  author={Kramers, Hendrik Anthony},
  journal={Physica},
  volume={7},
  number={4},
  pages={284--304},
  year={1940},
  publisher={Elsevier}
}
@article{bohr1939,
  title={The mechanism of nuclear fission},
  author={Bohr, Niels and Wheeler, John Archibald},
  journal={Physical Review},
  volume={56},
  number={5},
  pages={426},
  year={1939},
  publisher={APS}
}

@article{Monteoliva2000,
  title = {Decoherence and the Rate of Entropy Production in Chaotic Quantum Systems},
  author = {Monteoliva, Diana and Paz, Juan Pablo},
  journal = {Phys. Rev. Lett.},
  volume = {85},
  issue = {16},
  pages = {3373--3376},
  numpages = {0},
  year = {2000},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.85.3373},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.85.3373}
}

@book{Clarke2004,
   title =     {The SQUID Handbook: Fundamentals and Technology of SQUIDs and SQUID Systems},
   author =    {John Clarke, Alex I. Braginski},
   publisher = {Wiley-VCH},
   isbn =      {9783527402298,3527402292},
   year =      {2004},
   series =    {},
   edition =   {1},
   volume =    {},
   url =       {http://gen.lib.rus.ec/book/index.php?md5=0b337415287f031b98c6bac8edcdf5e1}
}

@article{puri2019,
  title = {Stabilized Cat in a Driven Nonlinear Cavity: A Fault-Tolerant Error Syndrome Detector},
  author = {Puri, Shruti and Grimm, Alexander and Campagne-Ibarcq, Philippe and Eickbusch, Alec and Noh, Kyungjoo and Roberts, Gabrielle and Jiang, Liang and Mirrahimi, Mazyar and Devoret, Michel H. and Girvin, S. M.},
  journal = {Phys. Rev. X},
  volume = {9},
  issue = {4},
  pages = {041009},
  numpages = {29},
  year = {2019},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevX.9.041009},
  url = {https://link.aps.org/doi/10.1103/PhysRevX.9.041009}
}


@Article{minev2019,
author={Minev, Z. K.
and Mundhada, S. O.
and Shankar, S.
and Reinhold, P.
and Guti{\'e}rrez-J{\'a}uregui, R.
and Schoelkopf, R. J.
and Mirrahimi, M.
and Carmichael, H. J.
and Devoret, M. H.},
title={To catch and reverse a quantum jump mid-flight},
journal={Nature},
year={2019},
month={Jun},
day={01},
volume={570},
number={7760},
pages={200-204},
abstract={},
issn={1476-4687},
doi={10.1038/s41586-019-1287-z},
url={https://doi.org/10.1038/s41586-019-1287-z}
}

@article{Nguyen2018,
  title = {Towards Quantum Simulation with Circular Rydberg Atoms},
  author = {Nguyen, T. L. and Raimond, J. M. and Sayrin, C. and Corti\~nas, R. and Cantat-Moltrecht, T. and Assemat, F. and Dotsenko, I. and Gleyzes, S. and Haroche, S. and Roux, G. and Jolicoeur, Th. and Brune, M.},
  journal = {Phys. Rev. X},
  volume = {8},
  issue = {1},
  pages = {011032},
  numpages = {27},
  year = {2018},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevX.8.011032},
  url = {https://link.aps.org/doi/10.1103/PhysRevX.8.011032}
}

@article{haroche2013,
  title = {Nobel Lecture: Controlling photons in a box and exploring the quantum to classical boundary},
  author = {Haroche, Serge},
  journal = {Rev. Mod. Phys.},
  volume = {85},
  issue = {3},
  pages = {1083--1102},
  numpages = {0},
  year = {2013},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/RevModPhys.85.1083},
  url = {https://link.aps.org/doi/10.1103/RevModPhys.85.1083}
}


@Article{Campagne-Ibarcq2020,
author={Campagne-Ibarcq, P.
and Eickbusch, A.
and Touzard, S.
and Zalys-Geller, E.
and Frattini, N. E.
and Sivak, V. V.
and Reinhold, P.
and Puri, S.
and Shankar, S.
and Schoelkopf, R. J.
and Frunzio, L.
and Mirrahimi, M.
and Devoret, M. H.},
title={Quantum error correction of a qubit encoded in grid states of an oscillator},
journal={Nature},
year={2020},
month={Aug},
day={01},
volume={584},
number={7821},
pages={368-372},
abstract={The accuracy of logical operations on quantum bits (qubits) must be improved for quantum computers to outperform classical ones in useful tasks. One method to achieve this is quantum error correction (QEC), which prevents noise in the underlying system from causing logical errors. This approach derives from the reasonable assumption that noise is local, that is, it does not act in a coordinated way on different parts of the physical system. Therefore, if a logical qubit is encoded non-locally, we can---for a limited time---detect and correct noise-induced evolution before it corrupts the encoded information1. In 2001, Gottesman, Kitaev and Preskill (GKP) proposed a hardware-efficient instance of such a non-local qubit: a superposition of position eigenstates that forms grid states of a single oscillator2. However, the implementation of measurements that reveal this noise-induced evolution of the oscillator while preserving the encoded information3--7 has proved to be experimentally challenging, and the only realization reported so far relied on post-selection8,9, which is incompatible with QEC. Here we experimentally prepare square and hexagonal GKP code states through a feedback protocol that incorporates non-destructive measurements that are implemented with a superconducting microwave cavity having the role of the oscillator. We demonstrate QEC of an encoded qubit with suppression of all logical errors, in quantitative agreement with a theoretical estimate based on the measured imperfections of the experiment. Our protocol is applicable to other continuous-variable systems and, in contrast to previous implementations of QEC10--14, can mitigate all logical errors generated by a wide variety of noise processes and facilitate fault-tolerant quantum computation.},
issn={1476-4687},
doi={10.1038/s41586-020-2603-3},
url={https://doi.org/10.1038/s41586-020-2603-3}
}

@article{kryuchkyan1996,
  title={Exact quantum theory of a parametrically driven dissipative anharmonic oscillator},
  author={Kryuchkyan, G Yu and Kheruntsyan, KV},
  journal={Optics communications},
  volume={127},
  number={4-6},
  pages={230--236},
  year={1996},
  publisher={Elsevier}
}


@book{dykman2012,
  title={Fluctuating nonlinear oscillators: from nanomechanics to quantum superconducting circuits},
  author={Dykman, Mark},
  year={2012},
  publisher={Oxford University Press}
}

@incollection{zurek1999,
  title={Why we don’t need quantum planetary dynamics: Decoherence and the correspondence principle for chaotic systems},
  author={Zurek, Wojciech Hubert and Paz, Juan Pablo},
  booktitle={Epistemological and Experimental Perspectives on Quantum Physics},
  pages={167--177},
  year={1999},
  publisher={Springer}
}


@Article{Goto2016,
author={Goto, Hayato},
title={Bifurcation-based adiabatic quantum computation with a nonlinear oscillator network},
journal={Scientific Reports},
year={2016},
month={Feb},
day={22},
volume={6},
number={1},
pages={21686},
abstract={The dynamics of nonlinear systems qualitatively change depending on their parameters, which is called bifurcation. A quantum-mechanical nonlinear oscillator can yield a quantum superposition of two oscillation states, known as a Schr{\"o}dinger cat state, via quantum adiabatic evolution through its bifurcation point. Here we propose a quantum computer comprising such quantum nonlinear oscillators, instead of quantum bits, to solve hard combinatorial optimization problems. The nonlinear oscillator network finds optimal solutions via quantum adiabatic evolution, where nonlinear terms are increased slowly, in contrast to conventional adiabatic quantum computation or quantum annealing, where quantum fluctuation terms are decreased slowly. As a result of numerical simulations, it is concluded that quantum superposition and quantum fluctuation work effectively to find optimal solutions. It is also notable that the present computer is analogous to neural computers, which are also networks of nonlinear components. Thus, the present scheme will open new possibilities for quantum computation, nonlinear science and artificial intelligence.},
issn={2045-2322},
doi={10.1038/srep21686},
url={https://doi.org/10.1038/srep21686}
}



@Unpublished{Venkat2022_delta,
  doi = {10.48550/ARXIV.2211.04605},
  
  url = {https://arxiv.org/abs/2211.04605},
  
  author = {Venkatraman, Jayameenakshi and Cortinas, Rodrigo G. and Frattini, Nicholas E. and Xiao, Xu and Devoret, Michel H.},
  
  keywords = {Quantum Physics (quant-ph), Mesoscale and Nanoscale Physics (cond-mat.mes-hall), Atomic Physics (physics.atom-ph), FOS: Physical sciences, FOS: Physical sciences},
  
  title = {Quantum interference of tunneling paths under a double-well barrier},
  
  publisher = {arXiv},
  
  year = {2022},
  eprint = {2211.04605},
  archivePrefix = "arXiv",
  primaryClass = "quant-ph",
}



@Article{Masuda2021,
author={Masuda, Shumpei
and Ishikawa, Toyofumi
and Matsuzaki, Yuichiro
and Kawabata, Shiro},
title={Controls of a superconducting quantum parametron under a strong pump field},
journal={Scientific Reports},
year={2021},
month={Jun},
day={01},
volume={11},
number={1},
pages={11459},
abstract={Pumped at approximately twice the natural frequency, a Josephson parametric oscillator called parametron or Kerr parametric oscillator shows self-oscillation. Quantum annealing and universal quantum computation using self-oscillating parametrons as qubits were proposed. However, controls of parametrons under the pump field are degraded by unwanted rapidly oscillating terms in the Hamiltonian, which we call non-resonant rapidly oscillating terms (NROTs) coming from the violation of the rotating wave approximation. Therefore, the pump field can be an intrinsic origin of the imperfection of controls of parametrons. Here, we theoretically study the influence of the NROTs on the accuracy of controls of a parametron: a cat-state creation and a single-qubit gate. It is shown that there is a trade-off relationship between the suppression of the nonadiabatic transitions and the validity of the rotating wave approximation in a conventional approach. We also show that the tailored time dependence of the detuning of the pump field can suppress both of the nonadiabatic transitions and the disturbance of the state of the parametron due to the NROTs.},
issn={2045-2322},
doi={10.1038/s41598-021-90874-4},
url={https://doi.org/10.1038/s41598-021-90874-4}
}




@article{BenStijnInPrep2022,
  title = {A high on-off ratio beamsplitter interaction for two-qubit gates on bosonically encoded qubits},
  author = {Chapman, Benjamin and de Graaf, Stijn  and Xue, Huayue and Schoelkof, Robert },
  journal = {In preparation},
  year = {2022},
}

@article{blais2004,
  title = {Cavity quantum electrodynamics for superconducting electrical circuits: An architecture for quantum computation},
  author = {Blais, Alexandre and Huang, Ren-Shou and Wallraff, Andreas and Girvin, S. M. and Schoelkopf, R. J.},
  journal = {Phys. Rev. A},
  volume = {69},
  issue = {6},
  pages = {062320},
  numpages = {14},
  year = {2004},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.69.062320},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.69.062320}
}


@article{BREUER1991249,
title = {A semiclassical theory of quasienergies and Floquet wave functions},
journal = {Annals of Physics},
volume = {211},
number = {2},
pages = {249-291},
year = {1991},
issn = {0003-4916},
doi = {https://doi.org/10.1016/0003-4916(91)90206-N},
url = {https://www.sciencedirect.com/science/article/pii/000349169190206N},
author = {H.P Breuer and M Holthaus},
abstract = {Employing the Maslov construction of the canonical operator, we derive semiclassical quantization rules for quasienergies and Floquet states of periodically time-dependent systems. The method is applied to a class of strongly driven anharmonic oscillators which, on the classical level, show a sharp division of the phase space into an almost regular and a stochastic region. For the almost regular part of motion the semiclassical quantization rules are shown to yield excellent approximations to the exact quantum mechanical quasienergies and Floquet states. The influence of resonances and stochastic motion on quasienergy spectra and Floquet wave functions is discussed. We demonstrate that an exact scaling relation valid for the classical Hamiltonian leads to an approximate scaling relation for the quasienergies which is broken in a characteristic manner by quantum effects.}
}




@article{kapitza1951,
	title={Dynamic stability of the pendulum with vibrating suspension point},
	author={Kapitza, PL},
	journal={Soviet Physics--JETP},
	volume={21},
	number={5},
	pages={588--597},
	year={1951}
}


@article{gammaitoni1998,
  title={Stochastic resonance},
  author={Gammaitoni, Luca and H{\"a}nggi, Peter and Jung, Peter and Marchesoni, Fabio},
  journal={Reviews of Modern Physics},
  volume={70},
  number={1},
  pages={223},
  year={1998},
  publisher={APS}
}

@book{bechhoefer2021,
  title={Control Theory for Physicists},
  author={Bechhoefer, John},
  year={2021},
  publisher={Cambridge University Press}
}

@book{landau1976,
  title={Mechanics: Volume 1},
  author={Landau, Lev Davidovich and Lifshitz, Evgenii Mikhailovich},
  volume={1},
  year={1976},
  publisher={Butterworth-Heinemann}
}


@article{wisdom1984,
  title={The chaotic rotation of Hyperion},
  author={Wisdom, Jack and Peale, Stanton J and Mignard, Fran{\c{c}}ois},
  journal={Icarus},
  volume={58},
  number={2},
  pages={137--152},
  year={1984},
  publisher={Elsevier}
}


@article{goldman2014,
  title={Periodically driven quantum systems: effective Hamiltonians and engineered gauge fields},
  author={Goldman, Nathan and Dalibard, Jean},
  journal={Phys. Rev. X},
  volume={4},
  number={3},
  pages={031027},
  year={2014},
  publisher={APS}
}

@article{wintersperger2020,
  title={Realization of an anomalous Floquet topological system with ultracold atoms},
  author={Wintersperger, Karen and Braun, Christoph and {\"U}nal, F Nur and Eckardt, Andr{\'e} and Di Liberto, Marco and Goldman, Nathan and Bloch, Immanuel and Aidelsburger, Monika},
  journal={Nature Physics},
  volume={16},
  number={10},
  pages={1058--1063},
  year={2020},
  publisher={Nature Publishing Group}
}

@article{brune1996,
  title = {Observing the Progressive Decoherence of the ``Meter'' in a Quantum Measurement},
  author = {Brune, M. and Hagley, E. and Dreyer, J. and Ma\^{\i}tre, X. and Maali, A. and Wunderlich, C. and Raimond, J. M. and Haroche, S.},
  journal = {Phys. Rev. Lett.},
  volume = {77},
  issue = {24},
  pages = {4887--4890},
  numpages = {0},
  year = {1996},
  month = {Dec},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.77.4887},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.77.4887}
}
@book{haroche2006,
  title={Exploring the quantum: atoms, cavities, and photons},
  author={Haroche, Serge and Raimond, J-M},
  year={2006},
  publisher={Oxford University Press}
}

@article{Blais2021,
  title = {Circuit quantum electrodynamics},
  author = {Blais, Alexandre and Grimsmo, Arne L. and Girvin, S. M. and Wallraff, Andreas},
  journal = {Rev. Mod. Phys.},
  volume = {93},
  issue = {2},
  pages = {025005},
  numpages = {72},
  year = {2021},
  month = {May},
  publisher = {American Physical Society},
  doi = {10.1103/RevModPhys.93.025005},
  url = {https://link.aps.org/doi/10.1103/RevModPhys.93.025005}
}


@article{Dalibard1985,
author = {J. Dalibard and C. Cohen-Tannoudji},
journal = {J. Opt. Soc. Am. B},
keywords = {Electric fields; Laser beams; Laser light; Radiation pressure; Resonance fluorescence; Spontaneous emission},
number = {11},
pages = {1707--1720},
publisher = {OSA},
title = {Dressed-atom approach to atomic motion in laser light: the dipole force revisited},
volume = {2},
month = {Nov},
year = {1985},
url = {http://opg.optica.org/josab/abstract.cfm?URI=josab-2-11-1707},
doi = {10.1364/JOSAB.2.001707},
}


@article{ribeiro2008,
  title = {Exact spectrum of the Lipkin-Meshkov-Glick model in the thermodynamic limit and finite-size corrections},
  author = {Ribeiro, Pedro and Vidal, Julien and Mosseri, R\'emy},
  journal = {Phys. Rev. E},
  volume = {78},
  issue = {2},
  pages = {021106},
  numpages = {13},
  year = {2008},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevE.78.021106},
  url = {https://link.aps.org/doi/10.1103/PhysRevE.78.021106}
}


@book{Frattini2021,
Author = {Nicholas E. Frattini},
Publisher = {Yale University, thesis},
Title = {Three-wave Mixing in Superconducting Circuits: Stabilizing Cats with SNAILs},
Year = {2021}
}

@article{Xiao2022,
author = {X. Xiao, and J. Venkatraman},
journal = {In preparation},
keywords = {},
number = {},
pages = {},
publisher = {},
title = {In preparation},
volume = {},
month = {},
year = {2022},
url = {},
doi = {},
}

@Unpublished{Shillito2022,
  doi = {10.48550/ARXIV.2203.11235},
  
  url = {https://arxiv.org/abs/2203.11235},
  
  author = {Shillito, Ross and Petrescu, Alexandru and Cohen, Joachim and Beall, Jackson and Hauru, Markus and Ganahl, Martin and Lewis, Adam G. M. and Vidal, Guifre and Blais, Alexandre},
  
  keywords = {Quantum Physics (quant-ph), FOS: Physical sciences, FOS: Physical sciences},
  
  title = {Dynamics of Transmon Ionization},
  
  publisher = {arXiv},
  
  year = {2022},
  eprint = {2203.11235},
  archivePrefix = "arXiv",
  primaryClass = "quant-ph",
}





@article{marthaler2007,
  title = {Quantum interference in the classically forbidden region: A parametric oscillator},
  author = {Marthaler, M. and Dykman, M. I.},
  journal = {Phys. Rev. A},
  volume = {76},
  issue = {1},
  pages = {010102},
  numpages = {4},
  year = {2007},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.76.010102},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.76.010102}
}


@article{Cohen1969,
author = {C. Cohen-Tannoudji and S. Haroche},
journal = {J. Phys. France},
number = {30},
pages = {153--168},
title = {Absorption et diffusion de photons optiques par un atome en interaction avec des photons de radiofréquence},
year = {1969},
url = {https://jphys.journaldephysique.org/articles/jphys/abs/1969/02/jphys_1969__30_2-3_153_0/jphys_1969__30_2-3_153_0.html},
doi = {10.1051/jphys:01969003002-3015300},
}

@book{landau2013quantum,
  title={Quantum mechanics: non-relativistic theory},
  author={Landau, Lev Davidovich and Lifshitz, Evgenii Mikhailovich},
  volume={3},
  year={2013},
  publisher={Elsevier}
}

@article{Zurek2003,
  title = {Decoherence, einselection, and the quantum origins of the classical},
  author = {Zurek, Wojciech Hubert},
  journal = {Rev. Mod. Phys.},
  volume = {75},
  issue = {3},
  pages = {715--775},
  numpages = {0},
  year = {2003},
  month = {May},
  publisher = {American Physical Society},
  doi = {10.1103/RevModPhys.75.715},
  url = {https://link.aps.org/doi/10.1103/RevModPhys.75.715}
}

@article{Leghtas2013,
  title = {Hardware-Efficient Autonomous Quantum Memory Protection},
  author = {Leghtas, Zaki and Kirchmair, Gerhard and Vlastakis, Brian and Schoelkopf, Robert J. and Devoret, Michel H. and Mirrahimi, Mazyar},
  journal = {Phys. Rev. Lett.},
  volume = {111},
  issue = {12},
  pages = {120501},
  numpages = {5},
  year = {2013},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.111.120501},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.111.120501}
}


@Article{kirchmair2013,
author={Kirchmair, Gerhard
and Vlastakis, Brian
and Leghtas, Zaki
and Nigg, Simon E.
and Paik, Hanhee
and Ginossar, Eran
and Mirrahimi, Mazyar
and Frunzio, Luigi
and Girvin, S. M.
and Schoelkopf, R. J.},
title={Observation of quantum state collapse and revival due to the single-photon Kerr effect},
journal={Nature},
year={2013},
month={Mar},
day={01},
volume={495},
number={7440},
pages={205-209},
abstract={An artificial Kerr medium has been engineered using superconducting circuits, enabling the observation of the characteristic collapse and revival of a coherent state; this behaviour could, for example, be used in single-photon generation and quantum logic operations.},
issn={1476-4687},
doi={10.1038/nature11902},
url={https://doi.org/10.1038/nature11902}
}




@article{touzard2018,
  title = {Coherent Oscillations inside a Quantum Manifold Stabilized by Dissipation},
  author = {Touzard, S. and Grimm, A. and Leghtas, Z. and Mundhada, S. O. and Reinhold, P. and Axline, C. and Reagor, M. and Chou, K. and Blumoff, J. and Sliwa, K. M. and Shankar, S. and Frunzio, L. and Schoelkopf, R. J. and Mirrahimi, M. and Devoret, M. H.},
  journal = {Phys. Rev. X},
  volume = {8},
  issue = {2},
  pages = {021005},
  numpages = {7},
  year = {2018},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevX.8.021005},
  url = {https://link.aps.org/doi/10.1103/PhysRevX.8.021005}
}

@article{deleglise2008,
  title={Reconstruction of non-classical cavity field states with snapshots of their decoherence},
  author={Deleglise, Samuel and Dotsenko, Igor and Sayrin, Clement and Bernu, Julien and Brune, Michel and Raimond, Jean-Michel and Haroche, Serge},
  journal={Nature},
  volume={455},
  number={7212},
  pages={510--514},
  year={2008},
  publisher={Nature Publishing Group}
}

@article{leghtas2015,
  title={Confining the state of light to a quantum manifold by engineered two-photon loss},
  author={Leghtas, Zaki and Touzard, Steven and Pop, Ioan M and Kou, Angela and Vlastakis, Brian and Petrenko, Andrei and Sliwa, Katrina M and Narla, Anirudh and Shankar, Shyam and Hatridge, Michael J and others},
  journal={Science},
  volume={347},
  number={6224},
  pages={853--857},
  year={2015},
  publisher={American Association for the Advancement of Science}
}


@article{grimm2020,
  title={Stabilization and operation of a Kerr-cat qubit},
  author={Grimm, Alexander and Frattini, Nicholas E and Puri, Shruti and Mundhada, Shantanu O and Touzard, Steven and Mirrahimi, Mazyar and Girvin, Steven M and Shankar, Shyam and Devoret, Michel H},
  journal={Nature},
  volume={584},
  number={7820},
  pages={205--209},
  year={2020},
  publisher={Nature Publishing Group}
}

@article{dirac1945,
  title={On the analogy between classical and quantum mechanics},
  author={Dirac, Paul Adrien Maurice},
  journal={Reviews of Modern Physics},
  volume={17},
  number={2-3},
  pages={195},
  year={1945},
  publisher={APS}
}

@Article{ofek2016,
author={Ofek, Nissim
and Petrenko, Andrei
and Heeres, Reinier
and Reinhold, Philip
and Leghtas, Zaki
and Vlastakis, Brian
and Liu, Yehan
and Frunzio, Luigi
and Girvin, S. M.
and Jiang, L.
and Mirrahimi, Mazyar
and Devoret, M. H.
and Schoelkopf, R. J.},
title={Extending the lifetime of a quantum bit with error correction in superconducting circuits},
journal={Nature},
year={2016},
month={Aug},
day={01},
volume={536},
number={7617},
pages={441-445},
abstract={A quantum-error-correction system is demonstrated in which natural errors due to energy loss are suppressed by encoding a logical state as a superposition of Schr{\"o}dinger-cat states, which results in the system reaching the `break-even' point, at which the lifetime of a qubit exceeds the lifetime of the constituents of the system.},
issn={1476-4687},
doi={10.1038/nature18949},
url={https://doi.org/10.1038/nature18949}
}

@article{Hsiao2020,
  title = {Efficient Orthogonal Control of Tunnel Couplings in a Quantum Dot Array},
  author = {Hsiao, T.-K. and van Diepen, C.J. and Mukhopadhyay, U. and Reichl, C. and Wegscheider, W. and Vandersypen, L.M.K.},
  journal = {Phys. Rev. Applied},
  volume = {13},
  issue = {5},
  pages = {054018},
  numpages = {9},
  year = {2020},
  month = {May},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevApplied.13.054018},
  url = {https://link.aps.org/doi/10.1103/PhysRevApplied.13.054018}
}

@article{vanHove1953,
  title = {The Occurrence of Singularities in the Elastic Frequency Distribution of a Crystal},
  author = {Van Hove, L\'eon},
  journal = {Phys. Rev.},
  volume = {89},
  issue = {6},
  pages = {1189--1193},
  numpages = {0},
  year = {1953},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRev.89.1189},
  url = {https://link.aps.org/doi/10.1103/PhysRev.89.1189}
}


@article{Alexandradinata2017,
  title = {Geometric Phase and Orbital Moment in Quantization Rules for Magnetic Breakdown},
  author = {Alexandradinata, A. and Glazman, Leonid},
  journal = {Phys. Rev. Lett.},
  volume = {119},
  issue = {25},
  pages = {256601},
  numpages = {6},
  year = {2017},
  month = {Dec},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.119.256601},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.119.256601}
}

@misc{Frattini2022,
  doi = {10.48550/ARXIV.2209.03934},
  
  url = {https://arxiv.org/abs/2209.03934},
  
  author = {Frattini, Nicholas E. and Cortiñas, Rodrigo G. and Venkatraman, Jayameenakshi and Xiao, Xu and Su, Qile and Lei, Chan U and Chapman, Benjamin J. and Joshi, Vidul R. and Girvin, S. M. and Schoelkopf, Robert J. and Puri, Shruti and Devoret, Michel H.},
  
  keywords = {Quantum Physics (quant-ph), FOS: Physical sciences, FOS: Physical sciences},
  
  title = {The squeezed Kerr oscillator: spectral kissing and phase-flip robustness},
  
  publisher = {arXiv},
  
  year = {2022},
  
  copyright = {Creative Commons Attribution 4.0 International}
}


@Unpublished{JXRnote,
  doi = {10.48550/ARXIV.2209.11193},
  
  url = {https://arxiv.org/abs/2209.11193},
  
  author = {Venkatraman, Jayameenakshi and Xiao, Xu and Cortiñas, Rodrigo G. and Devoret, Michel H.},
  
  keywords = {Quantum Physics (quant-ph), Mesoscale and Nanoscale Physics (cond-mat.mes-hall), Atomic Physics (physics.atom-ph), FOS: Physical sciences, FOS: Physical sciences},
  
  title = {On the static effective Lindbladian of the squeezed Kerr oscillator},
  
  year = {2022},
  eprint = {2209.11193},
  archivePrefix = "arXiv",
  primaryClass = "quant-ph",
}



@Article{Zheng2017,
author={Zheng, Hao
and Zhang, Junyi
and Berndt, Richard},
title={A minimal double quantum dot},
journal={Scientific Reports},
year={2017},
month={Sep},
day={07},
volume={7},
number={1},
pages={10764},
abstract={Double quantum dots (DQDs) are a versatile platform for solid-state physics, quantum computation and nanotechnology. The micro-fabrication techniques commonly used to fabricate DQDs are difficult to extend to the atomic scale. Using an alternative approach, which relies on scanning tunneling microscopy and spectroscopy, we prepared a minimal DQD in a wide band-gap semiconductor matrix. It is comprised of a pair of strongly coupled donor atoms that can each be doubly charged. The donor excitation diagram of this system mimicks the charge stability diagram observed in transport measurements of DQDs. We furthermore illustrate how the charge and spin degrees of freedom of the minimal DQD may be used to obtain a single quantum bit and to prepare a Bell state. The results open an intriguing perspective for quantum electronics with atomic-scale structures.},
issn={2045-2322},
doi={10.1038/s41598-017-10814-z},
url={https://doi.org/10.1038/s41598-017-10814-z}
}


@Article{Signoles2014,
author={Signoles, Adrien
and Facon, Adrien
and Grosso, Dorian
and Dotsenko, Igor
and Haroche, Serge
and Raimond, Jean-Michel
and Brune, Michel
and Gleyzes, S{\'e}bastien},
title={Confined quantum Zeno dynamics of a watched atomic arrow},
journal={Nature Physics},
year={2014},
month={Oct},
day={01},
volume={10},
number={10},
pages={715-719},
abstract={Repeatedly probing a quantum system restricts its evolution, providing a route for state engineering. Such confinement, described by quantum Zeno dynamics, has now been implemented to generate superposition states in a multi-level Rydberg atom.},
issn={1745-2481},
doi={10.1038/nphys3076},
url={https://doi.org/10.1038/nphys3076}
}


@Article{Andersen2020,
author={Andersen, Christian Kraglund
and Remm, Ants
and Lazar, Stefania
and Krinner, Sebastian
and Lacroix, Nathan
and Norris, Graham J.
and Gabureac, Mihai
and Eichler, Christopher
and Wallraff, Andreas},
title={Repeated quantum error detection in a surface code},
journal={Nature Physics},
year={2020},
month={Aug},
day={01},
volume={16},
number={8},
pages={875-880},
issn={1745-2481},
doi={10.1038/s41567-020-0920-y},
url={https://doi.org/10.1038/s41567-020-0920-y}
}




@article{stone2005,
author = {Stone,A. Douglas },
title = {Einstein’s Unknown Insight and the Problem of Quantizing Chaos},
journal = {Physics Today},
volume = {58},
number = {8},
pages = {37-43},
year = {2005},
doi = {10.1063/1.2062917},
URL = { 
        https://doi.org/10.1063/1.2062917
},
eprint = { 
        https://doi.org/10.1063/1.2062917
}
}


@article{kuhr2016,
  title={Quantum-gas microscopes: a new tool for cold-atom quantum simulators},
  author={Kuhr, Stefan},
  journal={National Science Review},
  volume={3},
  number={2},
  pages={170--172},
  year={2016},
  publisher={Oxford University Press}
}

@article{vijayan2022,
  title={Scalable all-optical cold damping of levitated nanoparticles},
  author={Vijayan, Jayadev and Zhang, Zhao and Piotrowski, Johannes and Windey, Dominik and van der Laan, Fons and Frimmer, Martin and Novotny, Lukas},
  journal={Nature Nanotechnology},
  pages={1--6},
  year={2022},
  publisher={Nature Publishing Group}
}

@article{regal2008,
  title={Measuring nanomechanical motion with a microwave cavity interferometer},
  author={Regal, CA and Teufel, JD and Lehnert, KW},
  journal={Nature Physics},
  volume={4},
  number={7},
  pages={555--560},
  year={2008},
  publisher={Nature Publishing Group UK London}
}

@article{Novotny2017,
  title = {Radiation damping of a polarizable particle},
  author = {Novotny, Lukas},
  journal = {Phys. Rev. A},
  volume = {96},
  issue = {3},
  pages = {032108},
  numpages = {5},
  year = {2017},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.96.032108},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.96.032108}
}


@article{Assemat2019,
  title = {Quantum Rabi Oscillations in Coherent and in Mesoscopic Cat Field States},
  author = {Assemat, F. and Grosso, D. and Signoles, A. and Facon, A. and Dotsenko, I. and Haroche, S. and Raimond, J. M. and Brune, M. and Gleyzes, S.},
  journal = {Phys. Rev. Lett.},
  volume = {123},
  issue = {14},
  pages = {143605},
  numpages = {5},
  year = {2019},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.123.143605},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.123.143605}
}


@article{Schymik2021,
  title = {Single Atoms with 6000-Second Trapping Lifetimes in Optical-Tweezer Arrays at Cryogenic Temperatures},
  author = {Schymik, Kai-Niklas and Pancaldi, Sara and Nogrette, Florence and Barredo, Daniel and Paris, Julien and Browaeys, Antoine and Lahaye, Thierry},
  journal = {Phys. Rev. Appl.},
  volume = {16},
  issue = {3},
  pages = {034013},
  numpages = {8},
  year = {2021},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevApplied.16.034013},
  url = {https://link.aps.org/doi/10.1103/PhysRevApplied.16.034013}
}


@article{young2020,
  title={Half-minute-scale atomic coherence and high relative stability in a tweezer clock},
  author={Young, Aaron W and Eckner, William J and Milner, William R and Kedar, Dhruv and Norcia, Matthew A and Oelker, Eric and Schine, Nathan and Ye, Jun and Kaufman, Adam M},
  journal={Nature},
  volume={588},
  number={7838},
  pages={408--413},
  year={2020},
  publisher={Nature Publishing Group UK London}
}

@article{robens2017,
  title={High numerical aperture (NA= 0.92) objective lens for imaging and addressing of cold atoms},
  author={Robens, Carsten and Brakhane, Stefan and Alt, Wolfgang and Klei{\ss}ler, Felix and Meschede, Dieter and Moon, Geol and Ramola, Gautam and Alberti, Andrea},
  journal={Optics letters},
  volume={42},
  number={6},
  pages={1043--1046},
  year={2017},
  publisher={Optica Publishing Group}
}

@article{Dutta2000,
  title = {Ponderomotive Optical Lattice for Rydberg Atoms},
  author = {Dutta, S. K. and Guest, J. R. and Feldbaum, D. and Walz-Flannigan, A. and Raithel, G.},
  journal = {Phys. Rev. Lett.},
  volume = {85},
  issue = {26},
  pages = {5551--5554},
  numpages = {0},
  year = {2000},
  month = {Dec},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.85.5551},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.85.5551}
}



@article{hillery1984,
title = {Distribution functions in physics: Fundamentals},
journal = {Physics Reports},
volume = {106},
number = {3},
pages = {121-167},
year = {1984},
issn = {0370-1573},
author = {Hillery, M. and O'Connell, R.F. and Scully, M.O. and Wigner, E.P.}
}



@article{McCoy1932,
author = {Neal H. McCoy },
title = {On the Function in Quantum Mechanics Which Corresponds to a Given Function in Classical Mechanics},
journal = {Proceedings of the National Academy of Sciences},
volume = {18},
number = {11},
pages = {674-676},
year = {1932},
}


@article{Assemat2019,
  title = {Quantum Rabi Oscillations in Coherent and in Mesoscopic Cat Field States},
  author = {Assemat, F. and Grosso, D. and Signoles, A. and Facon, A. and Dotsenko, I. and Haroche, S. and Raimond, J. M. and Brune, M. and Gleyzes, S.},
  journal = {Phys. Rev. Lett.},
  volume = {123},
  issue = {14},
  pages = {143605},
  numpages = {5},
  year = {2019},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.123.143605},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.123.143605}
}



@article{shirley1965,
  title={Solution of the Schr{\"o}dinger equation with a Hamiltonian periodic in time},
  author={Shirley, Jon H},
  journal={Physical Review},
  volume={138},
  number={4B},
  pages={B979},
  year={1965},
  publisher={APS}
}

@article{lescanne2020,
  title={Exponential suppression of bit-flips in a qubit encoded in an oscillator},
  author={Lescanne, Rapha{\"e}l and Villiers, Marius and Peronnin, Th{\'e}au and Sarlette, Alain and Delbecq, Matthieu and Huard, Benjamin and Kontos, Takis and Mirrahimi, Mazyar and Leghtas, Zaki},
  journal={Nature Physics},
  volume={16},
  number={5},
  pages={509--513},
  year={2020},
  publisher={Nature Publishing Group}
}

@article{wilson2011,
  title={Observation of the dynamical Casimir effect in a superconducting circuit},
  author={Wilson, Christopher M and Johansson, G{\"o}ran and Pourkabirian, Arsalan and Simoen, Michael and Johansson, J Robert and Duty, Tim and Nori, Franco and Delsing, Per},
  journal={nature},
  volume={479},
  number={7373},
  pages={376--379},
  year={2011},
  publisher={Nature Publishing Group}
}

@Inbook{Keil2021,
author="Keil, Mark
and Machluf, Shimon
and Margalit, Yair
and Zhou, Zhifan
and Amit, Omer
and Dobkowski, Or
and Japha, Yonathan
and Moukouri, Samuel
and Rohrlich, Daniel
and Binstock, Zina
and Bar-Haim, Yaniv
and Givon, Menachem
and Groswasser, David
and Meir, Yigal
and Folman, Ron",
editor="Friedrich, Bretislav
and Schmidt-B{\"o}cking, Horst",
title="Stern-Gerlach Interferometry with the Atom Chip",
bookTitle="Molecular Beams in Physics and Chemistry: From Otto Stern's Pioneering Exploits to Present-Day Feats",
year="2021",
publisher="Springer International Publishing",
address="Cham",
pages="263--301",
}

@article{PRA_nori2010,
  title = {Dynamical Casimir effect in superconducting microwave circuits},
  author = {Johansson, J. R. and Johansson, G. and Wilson, C. M. and Nori, Franco},
  journal = {Phys. Rev. A},
  volume = {82},
  issue = {5},
  pages = {052509},
  numpages = {17},
  year = {2010},
  month = {Nov},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.82.052509},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.82.052509}
}


@article{Shumeiko_Wallquist2006,
  title = {Selective coupling of superconducting charge qubits mediated by a tunable stripline cavity},
  author = {Wallquist, M. and Shumeiko, V. S. and Wendin, G.},
  journal = {Phys. Rev. B},
  volume = {74},
  issue = {22},
  pages = {224506},
  numpages = {10},
  year = {2006},
  month = {Dec},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.74.224506},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.74.224506}
}



@article{gerlich2011,
  title={Quantum interference of large organic molecules},
  author={Gerlich, Stefan and Eibenberger, Sandra and Tomandl, Mathias and Nimmrichter, Stefan and Hornberger, Klaus and Fagan, Paul J and T{\"u}xen, Jens and Mayor, Marcel and Arndt, Markus},
  journal={Nature communications},
  volume={2},
  number={1},
  pages={1--5},
  year={2011},
  publisher={Nature Publishing Group}
}

@article{Fluhmann2018,
  title = {Sequential Modular Position and Momentum Measurements of a Trapped Ion Mechanical Oscillator},
  author = {Fl\"uhmann, C. and Negnevitsky, V. and Marinelli, M. and Home, J. P.},
  journal = {Phys. Rev. X},
  volume = {8},
  issue = {2},
  pages = {021001},
  numpages = {17},
  year = {2018},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevX.8.021001},
  url = {https://link.aps.org/doi/10.1103/PhysRevX.8.021001}
}



@article{chamberland2020,
  title={Building a fault-tolerant quantum computer using concatenated cat codes},
  author={Chamberland, Christopher and Noh, Kyungjoo and Arrangoiz-Arriola, Patricio and Campbell, Earl T and Hann, Connor T and Iverson, Joseph and Putterman, Harald and Bohdanowicz, Thomas C and Flammia, Steven T and Keller, Andrew and others},
  journal={arXiv preprint arXiv:2012.04108},
  year={2020}
}


@article{Peano2012,
  title = {Sharp Tunneling Peaks in a Parametric Oscillator: Quantum Resonances Missing in the Rotating Wave Approximation},
  author = {Peano, V. and Marthaler, M. and Dykman, M. I.},
  journal = {Phys. Rev. Lett.},
  volume = {109},
  issue = {9},
  pages = {090401},
  numpages = {5},
  year = {2012},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.109.090401},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.109.090401}
}




@article{puri2017,
  title={Engineering the quantum states of light in a Kerr-nonlinear resonator by two-photon driving},
  author={Puri, Shruti and Boutin, Samuel and Blais, Alexandre},
  journal={npj Quantum Information},
  volume={3},
  number={1},
  pages={1--7},
  year={2017},
  publisher={Nature Publishing Group}
}

@article{yao2017,
  title={Discrete time crystals: Rigidity, criticality, and realizations},
  author={Yao, Norman Y and Potter, Andrew C and Potirniche, I-D and Vishwanath, Ashvin},
  journal={Phys. Rev. Lett.},
  volume={118},
  number={3},
  pages={030401},
  year={2017},
  publisher={APS}
}

@article{huang2018,
  title = {Clean Floquet Time Crystals: Models and Realizations in Cold Atoms},
  author = {Huang, Biao and Wu, Ying-Hai and Liu, W. Vincent},
  journal = {Phys. Rev. Lett.},
  volume = {120},
  issue = {11},
  pages = {110603},
  numpages = {7},
  year = {2018},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.120.110603}
}

@article{rylands2020,
  title = {Many-Body Dynamical Localization in a Kicked Lieb-Liniger Gas},
  author = {Rylands, Colin and Rozenbaum, Efim B. and Galitski, Victor and Konik, Robert},
  journal = {Phys. Rev. Lett.},
  volume = {124},
  issue = {15},
  pages = {155302},
  numpages = {6},
  year = {2020},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.124.155302}
}

@article{nandkishore2015,
  title={Many-body localization and thermalization in quantum statistical mechanics},
  author={Nandkishore, Rahul and Huse, David A},
  journal={Annu. Rev. Condens. Matter Phys.},
  volume={6},
  number={1},
  pages={15--38},
  year={2015},
  publisher={Annual Reviews}
}

@book{knapp1996,
  title={Lie groups beyond an introduction},
  author={Knapp, Anthony W and Knapp, AW},
  volume={140},
  year={1996},
  publisher={Springer}
}

@book{gilmore2008,
  title={Lie groups, physics, and geometry: an introduction for physicists, engineers and chemists},
  author={Gilmore, Robert},
  year={2008},
  publisher={Cambridge University Press}
}

@article{dragt1976,
  title={Lie series and invariant functions for analytic symplectic maps},
  author={Dragt, Alex J and Finn, John M},
  journal={Journal of Mathematical Physics},
  volume={17},
  number={12},
  pages={2215--2227},
  year={1976},
  publisher={American Institute of Physics}
}

@phdthesis{bukov2017,
  title={Floquet engineering in periodically driven closed quantum systems from dynamical localization to ultracold topological matter},
  author={Bukov, M},
  year={2017},
  school={Boston University}
}

@article{rahav2003,
  title = {Effective Hamiltonians for periodically driven systems},
  author = {Rahav, Saar and Gilary, Ido and Fishman, Shmuel},
  journal = {Phys. Rev. A},
  volume = {68},
  issue = {1},
  pages = {013820},
  numpages = {18},
  year = {2003},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.68.013820}
}

@article{eckardt2017,
  title={Colloquium: Atomic quantum gases in periodically driven optical lattices},
  author={Eckardt, Andr{\'e}},
  journal={Reviews of Modern Physics},
  volume={89},
  number={1},
  pages={011004},
  year={2017},
  publisher={APS}
}


@article{haeberlen1968,
  title={Coherent averaging effects in magnetic resonance},
  author={Haeberlen, U and Waugh, JS},
  journal={Phys. Rev.},
  volume={175},
  number={2},
  pages={453},
  year={1968},
  publisher={APS}
}

@article{deprit1969,
  title={Canonical transformations depending on a small parameter},
  author={Deprit, Andr{\'e}},
  journal={Celestial mechanics},
  volume={1},
  number={1},
  pages={12--30},
  year={1969},
  publisher={Springer}
}

@article{schrieffer1966,
  title = {Relation between the Anderson and Kondo Hamiltonians},
  author = {Schrieffer, J. R. and Wolff, P. A.},
  journal = {Phys. Rev.},
  volume = {149},
  issue = {2},
  pages = {491--492},
  numpages = {0},
  year = {1966},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRev.149.491},
}

@ARTICLE{bravyi2011,
  author = {Sergey Bravyi and David P. DiVincenzo and Daniel Loss},
  title = {Schrieffer-Wolff transformation for quantum many-body systems},
  journal = {Annals of Physics},
  year = {2011},
  volume = {326},
  pages = {2793-2826},
  number = {10},
  doi = {https://doi.org/10.1016/j.aop.2011.06.004},
  issn = {0003-4916},
  keywords = {Quantum many-body system, Perturbative expansion, Canonical transformation},
}


@ARTICLE{casas2001,
  author = {Casas, F and Oteo, J A and Ros, J},
  title = {{Floquet theory: exponential perturbative treatment}},
  journal = {Journal of Physics A, Mathematical and General},
  volume = {34},
  pages = {3379--3388},
  number = {16},
  address = {United Kingdom},
  issn = {0305-4470},
  year={2001},
}

@ARTICLE{eckardt2015,
  author = {Eckardt, Andr{\'e} and Anisimovas, Egidijus},
  title = {High-frequency approximation for periodically driven quantum systems
	from a Floquet-space perspective},
  journal = {New journal of physics},
  year = {2015},
  volume = {17},
  pages = {093039},
  number = {9},
  publisher = {IOP Publishing}
}


@article{mikami2016,
  title={Brillouin-Wigner theory for high-frequency expansion in periodically driven systems: Application to Floquet topological insulators},
  author={Mikami, Takahiro and Kitamura, Sota and Yasuda, Kenji and Tsuji, Naoto and Oka, Takashi and Aoki, Hideo},
  journal={Physical Review B},
  volume={93},
  number={14},
  pages={144307},
  year={2016},
  publisher={APS}
}

@book{nayfeh2008,
  title={Perturbation methods},
  author={Nayfeh, Ali H},
  year={2008},
  publisher={John Wiley \& Sons}
}

@article{nayfeh1980,
  title={Nonlinear oscillations},
  author={Nayfeh, Ali Hasan and Mook, Dean T and Holmes, P},
  year={1980}
}

@book{krylov1937,
  title = {Introduction to non-linear mechanics (In Russian)},
  publisher = {Ac. of Sci. Ukr. SSR},
  year = {1937},
  author = {Krylov, N. M. and Bogoliubov, N. N.},
  note = {[English translation by Princeton University Press, Princeton, 1947]}
}

@book{bogoliubov1961,
  title = {{Asymptotic methods in the theory of non-linear oscillations (In
	Russian)}},
  year = {1961},
  author = {Bogoliubov, N. N. and Mitropolsky, Y. A.},
  note = {[English translation by Hindustan Pub., Delhi, 1961; Gordon and Breach, New York, 1961]}
}

@ARTICLE{buishvili1979,
  author = {Buishvili, L L and Menabde, M G},
  title = {{Use of averaging method in problems of high-resolution nuclear magnetic
	resonance in solids}},
  journal = {Theoretical and Mathematical Physics},
  year = {1979},
  volume = {50},
  pages = {2435-2442},
  number = {6},
}

@book{mirrahimi2015,
  title={Dynamics and control of open quantum systems},
  author={Mirrahimi, Mazyar and Rouchon, Pierre},
  journal={Lecture notes},
  year={2015}
}

@article{shirley1965,
  title={Solution of the Schr{\"o}dinger equation with a Hamiltonian periodic in time},
  author={Shirley, Jon H},
  journal={Physical Review},
  volume={138},
  number={4B},
  pages={B979},
  year={1965},
  publisher={APS}
}

@incollection{groenewold1946,
  title={On the principles of elementary quantum mechanics},
  author={Groenewold, Hilbrand Johannes},
  booktitle={On the Principles of Elementary Quantum Mechanics},
  pages={1--56},
  year={1946},
  publisher={Springer}
}

@article{moyal1949, 
title={Quantum mechanics as a statistical theory}, 
volume={45}, 
DOI={10.1017/S0305004100000487}, 
number={1}, 
journal={Mathematical Proceedings of the Cambridge Philosophical Society}, 
publisher={Cambridge University Press}, 
author={Moyal, J. E.}, 
year={1949}, 
pages={99–124}}



@article{avan1976,
  title={Effect of high frequency irradiation on the dynamical properties of weakly bound electrons},
  author={Avan, P and Cohen-Tannoudji, C and Dupont-Roc, J and Fabre, C},
  journal={Journal de Physique},
  volume={37},
  number={9},
  pages={993--1009},
  year={1976},
  publisher={Soci{\'e}t{\'e} Fran{\c{c}}aise de Physique}
}

@article{hausinger2010,
  title={Dissipative two-level system under strong ac driving: A combination of floquet and van vleck perturbation theory},
  author={Hausinger, Johannes and Grifoni, Milena},
  journal={Physical Review A},
  volume={81},
  number={2},
  pages={022117},
  year={2010},
  publisher={APS}
}

@misc{vv2021,
  year = {2021},
  publisher = {GitHub},
  journal = {GitHub repository},
  howpublished = {\url{https://github.com/xiaoxuisaac/vanVleck-recursion}},
}

@article{xiao2021,
  title={Perturbative diagonalization for time-dependent strong interactions},
  author={Xiao, Z and Doucet, E and Noh, T and Ranzani, L and Simmonds, RW and Govia, LCG and Kamal, A},
  journal={arXiv preprint arXiv:2103.09260},
  year={2021}
}

@article{xiao2021_2,
author = {Xiao, Xu and Venkatraman, Jayameenakshi and Cortiñas, Rodrigo G. and Devoret, Michel H.},
journal = {in preparation},
year = {2021}}

@article{venkatraman2021,
    title={On the static effective Hamiltonian of a rapidly driven nonlinear system},
    author = {Venkatraman, Jayameenakshi and Xiao, Xu and Cortiñas, Rodrigo G. and Eickbusch, Alec and  Devoret, Michel H.},
    url = {https://doi.org/10.48550/arXiv.2108.02861},
    journal = {arXiv:2108.02861 [quant-ph]},
	month = aug,
    year = {2021}}

@article{zeuch2020,
author = {Zeuch, Daniel and Hassler, Fabian and Slim, Jesse J and DiVincenzo, David P},
doi = {https://doi.org/10.1016/j.aop.2020.168327},
issn = {0003-4916},
journal = {Annals of Physics},
keywords = { Beyond the rotating wave approximation, Magnus expansion, Stroboscopic time evolution, Strongly driven quantum system, Time-dependent perturbation theory,Quantum computation},
pages = {168327},
title = {{Exact rotating wave approximation}},
volume = {423},
year = {2020}
}


@article{petrescu2020,
  title = {Lifetime renormalization of driven weakly anharmonic superconducting qubits. II. The readout problem},
  author = {Petrescu, Alexandru and Malekakhlagh, Moein and T\"ureci, Hakan E.},
  journal = {Phys. Rev. B},
  volume = {101},
  issue = {13},
  pages = {134510},
  numpages = {27},
  year = {2020},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.101.134510}
}

@Unpublished{Masuda2022,
  doi = {10.48550/ARXIV.2203.00226},
  
  url = {https://arxiv.org/abs/2203.00226},
  
  author = {Masuda, Shumpei and Kanao, Taro and Goto, Hayato and Matsuzaki, Yuichiro and Ishikawa, Toyofumi and Kawabata, Shiro},
  
  keywords = {Quantum Physics (quant-ph), FOS: Physical sciences, FOS: Physical sciences},
  
  title = {Fast tunable coupling scheme of Kerr-nonlinear parametric oscillators based on shortcuts to adiabaticity},
  
  year = {2022},
  eprint = {2203.00226},
  archivePrefix = "arXiv",
  primaryClass = "quant-ph",
}

@article{Miyazaki2022,
	doi = {10.1103/physreva.105.062457},
  
	url = {https://doi.org/10.1103%2Fphysreva.105.062457},
  
	year = 2022,
	month = {jun},
  
	publisher = {American Physical Society ({APS})},
  
	volume = {105},
  
	number = {6},
  
	author = {Ryoji Miyazaki},
  
	title = {Effective spin models of Kerr-nonlinear parametric oscillators for quantum annealing},
  
	journal = {Physical Review A}
}


@Unpublished{Suzuki2022,
  doi = {10.48550/ARXIV.2208.04542},
  
  url = {https://arxiv.org/abs/2208.04542},
  
  author = {Suzuki, Yuta and Watabe, Shohei and Kawabata, Shiro and Masuda, Shumpei},
  
  keywords = {Quantum Physics (quant-ph), FOS: Physical sciences, FOS: Physical sciences},
  
  title = {Measurement-based state preparation of Kerr parametric oscillators},
  
  year = {2022},
  eprint = {2208.04542},
  archivePrefix = "arXiv",
  primaryClass = "quant-ph",
}


@Unpublished{Matsumoto2022,
  doi = {10.48550/ARXIV.2209.00909},
  
  url = {https://arxiv.org/abs/2209.00909},
  
  author = {Matsumoto, Keisuke and Yamaguchi, Aiko and Yamamoto, Tsuyoshi and Kawabata, Shiro and Matsuzaki, Yuichiro},
  
  keywords = {Quantum Physics (quant-ph), FOS: Physical sciences, FOS: Physical sciences},
  
  title = {Spectroscopic estimation of the photon number for superconducting Kerr parametric oscillators},
  
  year = {2022},
  eprint = {2209.00909},
  archivePrefix = "arXiv",
  primaryClass = "quant-ph",
}


@article{Wilson2010,
  title = {Photon Generation in an Electromagnetic Cavity with a Time-Dependent Boundary},
  author = {Wilson, C. M. and Duty, T. and Sandberg, M. and Persson, F. and Shumeiko, V. and Delsing, P.},
  journal = {Phys. Rev. Lett.},
  volume = {105},
  issue = {23},
  pages = {233907},
  numpages = {4},
  year = {2010},
  month = {Dec},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.105.233907},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.105.233907}
}


@Article{Kwon2022,
author={Kwon, Sangil
and Watabe, Shohei
and Tsai, Jaw-Shen},
title={Autonomous quantum error correction in a four-photon Kerr parametric oscillator},
journal={npj Quantum Information},
year={2022},
month={Apr},
day={22},
volume={8},
number={1},
pages={40},
abstract={Autonomous quantum error correction has gained considerable attention to avoid complicated measurements and feedback. Despite its simplicity compared with the conventional measurement-based quantum error correction, it is still a far from practical technique because of significant hardware overhead. We propose an autonomous quantum error correction scheme for a rotational symmetric bosonic code in a four-photon Kerr parametric oscillator. Our scheme is the simplest possible error correction scheme that can surpass the break-even point---it requires only a single continuous microwave tone. We also introduce an unconditional reset scheme that requires one more continuous microwave tone in addition to that for the error correction. The key properties underlying this simplicity are protected quasienergy states of a four-photon Kerr parametric oscillator and the degeneracy in its quasienergy level structure. These properties eliminate the need for state-by-state correction in the Fock basis. Our schemes greatly reduce the complexity of autonomous quantum error correction and thus may accelerate the use of the bosonic code for practical quantum computation.},
issn={2056-6387},
doi={10.1038/s41534-022-00553-z},
url={https://doi.org/10.1038/s41534-022-00553-z}
}




@article{Yamaji2022,
  title = {Spectroscopic observation of the crossover from a classical Duffing oscillator to a Kerr parametric oscillator},
  author = {Yamaji, T. and Kagami, S. and Yamaguchi, A. and Satoh, T. and Koshino, K. and Goto, H. and Lin, Z. R. and Nakamura, Y. and Yamamoto, T.},
  journal = {Phys. Rev. A},
  volume = {105},
  issue = {2},
  pages = {023519},
  numpages = {12},
  year = {2022},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.105.023519},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.105.023519}
}


@article{Frimmer2019,
  title = {Rapid Flipping of Parametric Phase States},
  author = {Frimmer, Martin and Heugel, Toni L. and Nosan, \ifmmode \check{Z}\else \v{Z}\fi{}iga and Tebbenjohanns, Felix and H\"alg, David and Akin, Abdulkadir and Degen, Christian L. and Novotny, Lukas and Chitra, R. and Zilberberg, Oded and Eichler, Alexander},
  journal = {Phys. Rev. Lett.},
  volume = {123},
  issue = {25},
  pages = {254102},
  numpages = {6},
  year = {2019},
  month = {Dec},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.123.254102},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.123.254102}
}



@Unpublished{Margiani2021,
  doi = {10.48550/ARXIV.2112.03357},
  
  url = {https://arxiv.org/abs/2112.03357},
  
  author = {Margiani, Gabriel and Guerrero, Sebastian and Heugel, Toni L. and Marty, Christian and Pachlatko, Raphael and Gisler, Thomas and Vukasin, Gabrielle D. and Kwon, Hyun-Keun and Miller, James ML. and Bousse, Nicholas E. and Kenny, Thomas W. and Zilberberg, Oded and Sabonis, Deividas and Eichler, Alexander},
  
  keywords = {Mesoscale and Nanoscale Physics (cond-mat.mes-hall), Chaotic Dynamics (nlin.CD), FOS: Physical sciences, FOS: Physical sciences},
  
  title = {Fluctuating Trajectories and Switching Rates of a Synthetic Two-Level System},
  
  year = {2021},
  eprint = {2112.03357},
  archivePrefix = "arXiv",
  primaryClass = "quant-ph",
}


@article{Qian2022,
  title = {Engineering fast bias-preserving gates on stabilized cat qubits},
  author = {Xu, Qian and Iverson, Joseph K. and Brand\~ao, Fernando G. S. L. and Jiang, Liang},
  journal = {Phys. Rev. Research},
  volume = {4},
  issue = {1},
  pages = {013082},
  numpages = {16},
  year = {2022},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevResearch.4.013082},
  url = {https://link.aps.org/doi/10.1103/PhysRevResearch.4.013082}
}


@article{Strandberg2021,
  title = {Wigner negativity in the steady-state output of a Kerr parametric oscillator},
  author = {Strandberg, Ingrid and Johansson, G\"oran and Quijandr\'{\i}a, Fernando},
  journal = {Phys. Rev. Research},
  volume = {3},
  issue = {2},
  pages = {023041},
  numpages = {13},
  year = {2021},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevResearch.3.023041},
  url = {https://link.aps.org/doi/10.1103/PhysRevResearch.3.023041}
}



@article{Ding2017,
  title = {Quantum Parametric Oscillator with Trapped Ions},
  author = {Ding, Shiqian and Maslennikov, Gleb and Habl\"utzel, Roland and Loh, Huanqian and Matsukevich, Dzmitry},
  journal = {Phys. Rev. Lett.},
  volume = {119},
  issue = {15},
  pages = {150404},
  numpages = {5},
  year = {2017},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.119.150404},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.119.150404}
}


@article{ZWang2019,
  title = {Quantum Dynamics of a Few-Photon Parametric Oscillator},
  author = {Wang, Zhaoyou and Pechal, Marek and Wollack, E. Alex and Arrangoiz-Arriola, Patricio and Gao, Maodong and Lee, Nathan R. and Safavi-Naeini, Amir H.},
  journal = {Phys. Rev. X},
  volume = {9},
  issue = {2},
  pages = {021049},
  numpages = {13},
  year = {2019},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevX.9.021049},
  url = {https://link.aps.org/doi/10.1103/PhysRevX.9.021049}
}

@article{Guillaud2019,
  title = {Repetition Cat Qubits for Fault-Tolerant Quantum Computation},
  author = {Guillaud, J\'er\'emie and Mirrahimi, Mazyar},
  journal = {Phys. Rev. X},
  volume = {9},
  issue = {4},
  pages = {041053},
  numpages = {23},
  year = {2019},
  month = {Dec},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevX.9.041053},
  url = {https://link.aps.org/doi/10.1103/PhysRevX.9.041053}
}

@article{mirrahimi2014,
  title={Dynamically protected cat-qubits: a new paradigm for universal quantum computation},
  author={Mirrahimi, Mazyar and Leghtas, Zaki and Albert, Victor V and Touzard, Steven and Schoelkopf, Robert J and Jiang, Liang and Devoret, Michel H},
  journal={New Journal of Physics},
  volume={16},
  number={4},
  pages={045014},
  year={2014},
  publisher={IOP Publishing}
}

@article{Fowler2012,
  title = {Surface codes: Towards practical large-scale quantum computation},
  author = {Fowler, Austin G. and Mariantoni, Matteo and Martinis, John M. and Cleland, Andrew N.},
  journal = {Phys. Rev. A},
  volume = {86},
  issue = {3},
  pages = {032324},
  numpages = {48},
  year = {2012},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.86.032324},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.86.032324}
}




@article{cochrane1999,
  title = {Macroscopically distinct quantum-superposition states as a bosonic code for amplitude damping},
  author = {Cochrane, P. T. and Milburn, G. J. and Munro, W. J.},
  journal = {Phys. Rev. A},
  volume = {59},
  issue = {4},
  pages = {2631--2634},
  numpages = {0},
  year = {1999},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.59.2631},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.59.2631}
}

@article{squeeze_states_param,
author = {Ling-An Wu and Min Xiao and H. J. Kimble},
journal = {J. Opt. Soc. Am. B},
keywords = {Optical parametric oscillators; Parametric down conversion; Parametric processes; Phase space analysis methods; Quantum fluctuations; Uncertainty principle},
number = {10},
pages = {1465--1475},
publisher = {Optica Publishing Group},
title = {Squeezed states of light from an optical parametric oscillator},
volume = {4},
month = {Oct},
year = {1987},
url = {https://opg.optica.org/josab/abstract.cfm?URI=josab-4-10-1465},
doi = {10.1364/JOSAB.4.001465},
abstract = {Squeezed states of the electromagnetic field are generated by degenerate parametric downconversion in a sub-threshold optical parametric oscillator. Reductions in photocurrent noise greater than 60\% ({\textminus}4 dB) below the limit set by the vacuum fluctuations of the field are observed in a balanced homodyne detector. A quantitative comparison with theory suggests that the observed noise reductions result from a field that in the absence of avoidable linear attenuation would be squeezed more than tenfold. A degree of squeezing of approximately fivefold is inferred for the actual field emitted through one mirror of the optical parametric oscillator. An explicit demonstration of the Heisenberg uncertainty principle for the electromagnetic field is made from the measurements, which show that the field state produced by the downconversion process is a state of minimum uncertainty.},
}

@article{millisecond2023,
  title = {Millisecond Coherence in a Superconducting Qubit},
  author = {Somoroff, Aaron and Ficheux, Quentin and Mencia, Raymond A. and Xiong, Haonan and Kuzmin, Roman and Manucharyan, Vladimir E.},
  journal = {Phys. Rev. Lett.},
  volume = {130},
  issue = {26},
  pages = {267001},
  numpages = {6},
  year = {2023},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.130.267001},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.130.267001}
}


@article{Gilchrist2004,
doi = {10.1088/1464-4266/6/8/032},
url = {https://dx.doi.org/10.1088/1464-4266/6/8/032},
year = {2004},
month = {jul},
publisher = {},
volume = {6},
number = {8},
pages = {S828},
author = {A Gilchrist and  Kae Nemoto and  W J Munro and  T C Ralph and  S Glancy and  Samuel L Braunstein and  G J Milburn},
title = {Schrödinger cats and their power for quantum information processing},
journal = {Journal of Optics B: Quantum and Semiclassical Optics},
abstract = {We outline a toolbox comprised of passive optical elements, single photon detection and superpositions of coherent states (Schrödinger cat states). Such a toolbox is a powerful collection of primitives for quantum information processing tasks. We illustrate its use by outlining a proposal for universal quantum computation. We utilize this toolbox for quantum metrology applications, for instance weak force measurements and precise phase estimation. We show in both these cases that a sensitivity at the Heisenberg limit is achievable.}
}

@article{milburn1991,
  title = {Quantum coherence and classical chaos in a pulsed parametric oscillator with a Kerr nonlinearity},
  author = {Milburn, G. J. and Holmes, C. A.},
  journal = {Phys. Rev. A},
  volume = {44},
  issue = {7},
  pages = {4704--4711},
  numpages = {0},
  year = {1991},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.44.4704},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.44.4704}
}

@article{milburn1986,
  title = {Dissipative Quantum and Classical Liouville Mechanics of the Anharmonic Oscillator},
  author = {Milburn, G. J. and Holmes, C. A.},
  journal = {Phys. Rev. Lett.},
  volume = {56},
  issue = {21},
  pages = {2237--2240},
  numpages = {0},
  year = {1986},
  month = {May},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.56.2237},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.56.2237}
}

@article{Goto2019,
author = {Goto ,Hayato},
title = {Quantum Computation Based on Quantum Adiabatic Bifurcations of Kerr-Nonlinear Parametric Oscillators},
journal = {Journal of the Physical Society of Japan},
volume = {88},
number = {6},
pages = {061015},
year = {2019},
doi = {10.7566/JPSJ.88.061015},

URL = { 
        https://doi.org/10.7566/JPSJ.88.061015
    
}
}



@article{Wang2013,
  title = {Coherent Ising machine based on degenerate optical parametric oscillators},
  author = {Wang, Zhe and Marandi, Alireza and Wen, Kai and Byer, Robert L. and Yamamoto, Yoshihisa},
  journal = {Phys. Rev. A},
  volume = {88},
  issue = {6},
  pages = {063853},
  numpages = {9},
  year = {2013},
  month = {Dec},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.88.063853},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.88.063853}
}


@article{wielinga1993,
  title = {Quantum tunneling in a Kerr medium with parametric pumping},
  author = {Wielinga, B. and Milburn, G. J.},
  journal = {Phys. Rev. A},
  volume = {48},
  issue = {3},
  pages = {2494--2496},
  numpages = {0},
  year = {1993},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.48.2494},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.48.2494}
}


@article{frattini2017,
  title={3-wave mixing Josephson dipole element},
  author={Frattini, NE and Vool, U and Shankar, S and Narla, A and Sliwa, KM and Devoret, MH},
  journal={Applied Physics Letters},
  volume={110},
  number={22},
  pages={222603},
  year={2017},
  publisher={AIP Publishing LLC}
}

@ARTICLE{Harris1969,
  author={Harris, S.E.},
  journal={Proceedings of the IEEE}, 
  title={Tunable optical parametric oscillators}, 
  year={1969},
  volume={57},
  number={12},
  pages={2096-2113},
  doi={10.1109/PROC.1969.7495}}
  
 @article{Kinsler1991,
  title = {Quantum dynamics of the parametric oscillator},
  author = {Kinsler, P. and Drummond, P. D.},
  journal = {Phys. Rev. A},
  volume = {43},
  issue = {11},
  pages = {6194--6208},
  numpages = {0},
  year = {1991},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.43.6194},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.43.6194}
}


@article{yurke1988,
title = {The dynamic generation of Schrödinger cats and their detection},
journal = {Physica B+C},
volume = {151},
number = {1},
pages = {298-301},
year = {1988},
issn = {0378-4363},
doi = {https://doi.org/10.1016/0378-4363(88)90181-7},
url = {https://www.sciencedirect.com/science/article/pii/0378436388901817},
author = {B. Yurke and D. Stoler},
abstract = {A coherent state interacting with a suitable nonlinearity can be transformed into a quantum superposition of two coherent states 180° out of phase with each other. The interference between the two macroscopic components of this Schrödinger's cat-like state can be detected with a homodyne detector.}
}

@article{yurke1986,
  title = {Generating quantum mechanical superpositions of macroscopically distinguishable states via amplitude dispersion},
  author = {Yurke, B. and Stoler, D.},
  journal = {Phys. Rev. Lett.},
  volume = {57},
  issue = {1},
  pages = {13--16},
  numpages = {0},
  year = {1986},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.57.13},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.57.13}
}

@article{aliferis2008,
  title = {Fault-tolerant quantum computation against biased noise},
  author = {Aliferis, Panos and Preskill, John},
  journal = {Phys. Rev. A},
  volume = {78},
  issue = {5},
  pages = {052331},
  numpages = {9},
  year = {2008},
  month = {Nov},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.78.052331},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.78.052331}
}

@article{aliferis2009,
  title={Fault-tolerant computing with biased-noise superconducting qubits: a case study},
  author={Aliferis, Panos and Brito, Frederico and DiVincenzo, David P and Preskill, John and Steffen, Matthias and Terhal, Barbara M},
  journal={New Journal of Physics},
  volume={11},
  number={1},
  pages={013061},
  year={2009},
  publisher={IOP Publishing}
}



@article{caprio2008,
title = {Excited state quantum phase transitions in many-body systems},
journal = {Annals of Physics},
volume = {323},
number = {5},
pages = {1106-1135},
year = {2008},
issn = {0003-4916},
doi = {https://doi.org/10.1016/j.aop.2007.06.011},
url = {https://www.sciencedirect.com/science/article/pii/S0003491607001042},
author = {M.A. Caprio and P. Cejnar and F. Iachello},
}

@article{zhang2017,
  title = {Preparing quasienergy states on demand: A parametric oscillator},
  author = {Zhang, Yaxing and Dykman, M. I.},
  journal = {Phys. Rev. A},
  volume = {95},
  issue = {5},
  pages = {053841},
  numpages = {10},
  year = {2017},
  month = {May},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.95.053841},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.95.053841}
  }
  
@Article{Wilson2011,
author={Wilson, C. M.
and Johansson, G.
and Pourkabirian, A.
and Simoen, M.
and Johansson, J. R.
and Duty, T.
and Nori, F.
and Delsing, P.},
title={Observation of the dynamical Casimir effect in a superconducting circuit},
journal={Nature},
year={2011},
month={Nov},
day={01},
volume={479},
number={7373},
pages={376-379},
issn={1476-4687},
doi={10.1038/nature10561},
url={https://doi.org/10.1038/nature10561}
}


@article{Dykman1998,
  title = {Fluctuational phase-flip transitions in parametrically driven oscillators},
  author = {Dykman, M. I. and Maloney, C. M. and Smelyanskiy, V. N. and Silverstein, M.},
  journal = {Phys. Rev. E},
  volume = {57},
  issue = {5},
  pages = {5202--5212},
  numpages = {0},
  year = {1998},
  month = {May},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevE.57.5202},
  url = {https://link.aps.org/doi/10.1103/PhysRevE.57.5202}
}


@book{dykmanBook2012,
  title     = "Fluctuating Nonlinear Oscillators: From Nanomechanics to Quantum Superconducting Circuits",
  author    = "Dykman, Mark",
  year      = 2012,
  publisher = "Oxford",
  url   = "DOI:10.1093/acprof:oso/9780199691388.001.0001"
}


@article{shillito2022,
  title={Dynamics of Transmon Ionization},
  author={Shillito, Ross and Petrescu, Alexandru and Cohen, Joachim and Beall, Jackson and Hauru, Markus and Ganahl, Martin and Lewis, Adam GM and Vidal, Guifre and Blais, Alexandre},
  journal={arXiv preprint arXiv:2203.11235},
  year={2022}
}


@article{Mundada2020,
  title = {Floquet-Engineered Enhancement of Coherence Times in a Driven Fluxonium Qubit},
  author = {Mundada, Pranav S. and Gyenis, Andr\'as and Huang, Ziwen and Koch, Jens and Houck, Andrew A.},
  journal = {Phys. Rev. Applied},
  volume = {14},
  issue = {5},
  pages = {054033},
  numpages = {13},
  year = {2020},
  month = {Nov},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevApplied.14.054033},
  url = {https://link.aps.org/doi/10.1103/PhysRevApplied.14.054033}
}



@article{Sank2016,
  title = {Measurement-Induced State Transitions in a Superconducting Qubit: Beyond the Rotating Wave Approximation},
  author = {Sank, Daniel and Chen, Zijun and Khezri, Mostafa and Kelly, J. and Barends, R. and Campbell, B. and Chen, Y. and Chiaro, B. and Dunsworth, A. and Fowler, A. and Jeffrey, E. and Lucero, E. and Megrant, A. and Mutus, J. and Neeley, M. and Neill, C. and O'Malley, P. J. J. and Quintana, C. and Roushan, P. and Vainsencher, A. and White, T. and Wenner, J. and Korotkov, Alexander N. and Martinis, John M.},
  journal = {Phys. Rev. Lett.},
  volume = {117},
  issue = {19},
  pages = {190503},
  numpages = {6},
  year = {2016},
  month = {Nov},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.117.190503},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.117.190503}
}


@article{barends2014,
  title={Superconducting quantum circuits at the surface code threshold for fault tolerance},
  author={Barends, Rami and Kelly, Julian and Megrant, Anthony and Veitia, Andrzej and Sank, Daniel and Jeffrey, Evan and White, Ted C and Mutus, Josh and Fowler, Austin G and Campbell, Brooks and others},
  journal={Nature},
  volume={508},
  number={7497},
  pages={500--503},
  year={2014},
  publisher={Nature Publishing Group}
}

@article{Arute2019,
  title={Quantum supremacy using a programmable superconducting processor},
  author={Arute, Frank and Arya, Kunal and Babbush, Ryan and Bacon, Dave and Bardin, Joseph C and Barends, Rami and Biswas, Rupak and Boixo, Sergio and Brandao, Fernando GSL and Buell, David A and others},
  journal={Nature},
  volume={574},
  number={7779},
  pages={505--510},
  year={2019},
  publisher={Nature Publishing Group}
}
@Unpublished{Krinner2021,
  doi = {10.48550/ARXIV.2112.03708},
  
  url = {https://arxiv.org/abs/2112.03708},
  
  author = {Krinner, Sebastian and Lacroix, Nathan and Remm, Ants and Di Paolo, Agustin and Genois, Elie and Leroux, Catherine and Hellings, Christoph and Lazar, Stefania and Swiadek, Francois and Herrmann, Johannes and Norris, Graham J. and Andersen, Christian Kraglund and Müller, Markus and Blais, Alexandre and Eichler, Christopher and Wallraff, Andreas},
  
  keywords = {Quantum Physics (quant-ph), Mesoscale and Nanoscale Physics (cond-mat.mes-hall), FOS: Physical sciences, FOS: Physical sciences},
  
  title = {Realizing Repeated Quantum Error Correction in a Distance-Three Surface Code},
  
  year = {2021},
  eprint = {2112.03708},
  archivePrefix = "arXiv",
  primaryClass = "quant-ph",
}


@Article{Chen2021,
author={Chen, Zijun and AI, Google Quantum},
title={Exponential suppression of bit or phase errors with cyclic error correction},
journal={Nature},
year={2021},
month={Jul},
day={01},
volume={595},
number={7867},
pages={383-387},
issn={1476-4687},
doi={10.1038/s41586-021-03588-y},
url={https://doi.org/10.1038/s41586-021-03588-y}
}


@article{Chernoguzov2021,
  title = {Realization of Real-Time Fault-Tolerant Quantum Error Correction},
  author = {Ryan-Anderson, C. and Bohnet, J. G. and Lee, K. and Gresh, D. and Hankin, A. and Gaebler, J. P. and Francois, D. and Chernoguzov, A. and Lucchetti, D. and Brown, N. C. and Gatterman, T. M. and Halit, S. K. and Gilmore, K. and Gerber, J. A. and Neyenhuis, B. and Hayes, D. and Stutz, R. P.},
  journal = {Phys. Rev. X},
  volume = {11},
  issue = {4},
  pages = {041058},
  numpages = {29},
  year = {2021},
  month = {Dec},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevX.11.041058},
  url = {https://link.aps.org/doi/10.1103/PhysRevX.11.041058}
}


@Article{Corcoles2015,
author={C{\'o}rcoles, A. D.
and Magesan, Easwar
and Srinivasan, Srikanth J.
and Cross, Andrew W.
and Steffen, M.
and Gambetta, Jay M.
and Chow, Jerry M.},
title={Demonstration of a quantum error detection code using a square lattice of four superconducting qubits},
journal={Nature Communications},
year={2015},
month={Apr},
day={29},
volume={6},
number={1},
pages={6979},
issn={2041-1723},
doi={10.1038/ncomms7979},
url={https://doi.org/10.1038/ncomms7979}
}









@article{Devoret2013,
author = {M. H. Devoret  and R. J. Schoelkopf },
title = {Superconducting Circuits for Quantum Information: An Outlook},
journal = {Science},
volume = {339},
number = {6124},
pages = {1169-1174},
year = {2013},
doi = {10.1126/science.1231930},
URL = {https://www.science.org/doi/abs/10.1126/science.1231930},
eprint = {https://www.science.org/doi/pdf/10.1126/science.1231930},
abstract = {The performance of superconducting qubits has improved by several orders of magnitude in the past decade. These circuits benefit from the robustness of superconductivity and the Josephson effect, and at present they have not encountered any hard physical limits. However, building an error-corrected information processor with many such qubits will require solving specific architecture problems that constitute a new field of research. For the first time, physicists will have to master quantum error correction to design and operate complex active systems that are dissipative in nature, yet remain coherent indefinitely. We offer a view on some directions for the field and speculate on its future.}}

@article{Touzard2019,
  title = {Gated Conditional Displacement Readout of Superconducting Qubits},
  author = {Touzard, S. and Kou, A. and Frattini, N. E. and Sivak, V. V. and Puri, S. and Grimm, A. and Frunzio, L. and Shankar, S. and Devoret, M. H.},
  journal = {Phys. Rev. Lett.},
  volume = {122},
  issue = {8},
  pages = {080502},
  numpages = {6},
  year = {2019},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.122.080502},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.122.080502}
}


@book{curtright2013,
  title={A concise treatise on quantum mechanics in phase space},
  author={Curtright, Thomas L and Fairlie, David B and Zachos, Cosmas K},
  year={2013},
  publisher={World Scientific Publishing Company}
}

@article{bonilla_ataides_xzzx_2021,
	title = {The {XZZX} surface code},
	volume = {12},
	copyright = {2021 The Author(s)},
	issn = {2041-1723},
	url = {https://www.nature.com/articles/s41467-021-22274-1},
	doi = {10.1038/s41467-021-22274-1},
	number = {1},
	urldate = {2021-09-05},
	journal = {Nature Communications},
	author = {Bonilla Ataides, J. Pablo and Tuckett, David K. and Bartlett, Stephen D. and Flammia, Steven T. and Brown, Benjamin J.},
	month = apr,
	year = {2021},
	pages = {2172},
}

@article{darmawan_practical_2021,
	title = {Practical {Quantum} {Error} {Correction} with the {XZZX} {Code} and {Kerr}-{Cat} {Qubits}},
	volume = {2},
	url = {https://link.aps.org/doi/10.1103/PRXQuantum.2.030345},
	doi = {10.1103/PRXQuantum.2.030345},
	number = {3},
	urldate = {2022-04-29},
	journal = {PRX Quantum},
	author = {Darmawan, Andrew S. and Brown, Benjamin J. and Grimsmo, Arne L. and Tuckett, David K. and Puri, Shruti},
	month = sep,
	year = {2021},
	note = {Publisher: American Physical Society},
	pages = {030345},
}

@article{gyenis_moving_2021,
	title = {Moving beyond the {Transmon}: {Noise}-{Protected} {Superconducting} {Quantum} {Circuits}},
	volume = {2},
	shorttitle = {Moving beyond the {Transmon}},
	url = {https://link.aps.org/doi/10.1103/PRXQuantum.2.030101},
	doi = {10.1103/PRXQuantum.2.030101},
	number = {3},
	urldate = {2021-09-09},
	journal = {PRX Quantum},
	author = {Gyenis, András and Di Paolo, Agustin and Koch, Jens and Blais, Alexandre and Houck, Andrew A. and Schuster, David I.},
	month = sep,
	year = {2021},
	note = {Publisher: American Physical Society},
	pages = {030101},
}

@article{mi_time-crystalline_2021,
	title = {Time-{Crystalline} {Eigenstate} {Order} on a {Quantum} {Processor}},
	copyright = {2021 The Author(s), under exclusive licence to Springer Nature Limited},
	issn = {1476-4687},
	url = {https://www.nature.com/articles/s41586-021-04257-w},
	doi = {10.1038/s41586-021-04257-w},
	language = {english},
	urldate = {2021-12-01},
	journal = {Nature},
	author = {Mi, Xiao and Ippoliti, Matteo and Quintana, Chris and Greene, Ami and Chen, Zijun and Gross, Jonathan and Arute, Frank and Arya, Kunal and Atalaya, Juan and Babbush, Ryan and Bardin, Joseph C. and Basso, Joao and Bengtsson, Andreas and Bilmes, Alexander and Bourassa, Alexandre and Brill, Leon and Broughton, Michael and Buckley, Bob B. and Buell, David A. and Burkett, Brian and Bushnell, Nicholas and Chiaro, Benjamin and Collins, Roberto and Courtney, William and Debroy, Dripto and Demura, Sean and Derk, Alan R. and Dunsworth, Andrew and Eppens, Daniel and Erickson, Catherine and Farhi, Edward and Fowler, Austin G. and Foxen, Brooks and Gidney, Craig and Giustina, Marissa and Harrigan, Matthew P. and Harrington, Sean D. and Hilton, Jeremy and Ho, Alan and Hong, Sabrina and Huang, Trent and Huff, Ashley and Huggins, William J. and Ioffe, L. B. and Isakov, Sergei V. and Iveland, Justin and Jeffrey, Evan and Jiang, Zhang and Jones, Cody and Kafri, Dvir and Khattar, Tanuj and Kim, Seon and Kitaev, Alexei and Klimov, Paul V. and Korotkov, Alexander N. and Kostritsa, Fedor and Landhuis, David and Laptev, Pavel and Lee, Joonho and Lee, Kenny and Locharla, Aditya and Lucero, Erik and Martin, Orion and McClean, Jarrod R. and McCourt, Trevor and McEwen, Matt and Miao, Kevin C. and Mohseni, Masoud and Montazeri, Shirin and Mruczkiewicz, Wojciech and Naaman, Ofer and Neeley, Matthew and Neill, Charles and Newman, Michael and Niu, Murphy Yuezhen and O’Brien, Thomas E. and Opremcak, Alex and Ostby, Eric and Pato, Balint and Petukhov, Andre and Rubin, Nicholas C. and Sank, Daniel and Satzinger, Kevin J. and Shvarts, Vladimir and Su, Yuan and Strain, Doug and Szalay, Marco and Trevithick, Matthew D. and Villalonga, Benjamin and White, Theodore and Yao, Z. Jamie and Yeh, Ping and Yoo, Juhwan and Zalcman, Adam and Neven, Hartmut and Boixo, Sergio and Smelyanskiy, Vadim and Megrant, Anthony and Kelly, Julian and Chen, Yu and Sondhi, S. L. and Moessner, Roderich and Kechedzhi, Kostyantyn and Khemani, Vedika and Roushan, Pedram},
	month = nov,
	year = {2021},
}

@article{Schymik2021,
  title = {Single Atoms with 6000-Second Trapping Lifetimes in Optical-Tweezer Arrays at Cryogenic Temperatures},
  author = {Schymik, Kai-Niklas and Pancaldi, Sara and Nogrette, Florence and Barredo, Daniel and Paris, Julien and Browaeys, Antoine and Lahaye, Thierry},
  journal = {Phys. Rev. Appl.},
  volume = {16},
  issue = {3},
  pages = {034013},
  numpages = {8},
  year = {2021},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevApplied.16.034013},
  url = {https://link.aps.org/doi/10.1103/PhysRevApplied.16.034013}
}


@article{Ravon2023,
    author  = {Brice Ravon}, 
    year    = {2023},
    journal = {In preparation},
}

@article{Lachaude2023,
    author  = {Léa Lachaude}, 
    year    = {2023},
    journal = {In preparation},
}
    
@article{Barredo2020,
  title = {Three-Dimensional Trapping of Individual Rydberg Atoms in Ponderomotive Bottle Beam Traps},
  author = {Barredo, D. and Lienhard, V. and Scholl, P. and de L\'es\'eleuc, S. and Boulier, T. and Browaeys, A. and Lahaye, T.},
  journal = {Phys. Rev. Lett.},
  volume = {124},
  issue = {2},
  pages = {023201},
  numpages = {6},
  year = {2020},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.124.023201},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.124.023201}
}


@article{Wu2023,
	doi = {10.1103/physrevlett.130.023202},
  
	url = {https://doi.org/10.1103%2Fphysrevlett.130.023202},
  
	year = 2023,
	month = {jan},
  
	publisher = {American Physical Society ({APS})},
  
	volume = {130},
  
	number = {2},
  
	author = {H. Wu and R. Richaud and J.-M. Raimond and M. Brune and S. Gleyzes},
  
	title = {Millisecond-Lived Circular Rydberg Atoms in a Room-Temperature Experiment},
  
	journal = {Physical Review Letters}
}


@article{Cantat2020,
  title = {Long-lived circular Rydberg states of laser-cooled rubidium atoms in a cryostat},
  author = {Cantat-Moltrecht, T. and Corti\~nas, R. and Ravon, B. and M\'ehaignerie, P. and Haroche, S. and Raimond, J. M. and Favier, M. and Brune, M. and Sayrin, C.},
  journal = {Phys. Rev. Res.},
  volume = {2},
  issue = {2},
  pages = {022032},
  numpages = {6},
  year = {2020},
  month = {May},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevResearch.2.022032},
  url = {https://link.aps.org/doi/10.1103/PhysRevResearch.2.022032}
}


@article{Cortinas2020,
  title = {Laser Trapping of Circular Rydberg Atoms},
  author = {Corti\~nas, R. G. and Favier, M. and Ravon, B. and M\'ehaignerie, P. and Machu, Y. and Raimond, J. M. and Sayrin, C. and Brune, M.},
  journal = {Phys. Rev. Lett.},
  volume = {124},
  issue = {12},
  pages = {123201},
  numpages = {6},
  year = {2020},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.124.123201},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.124.123201}
}


@article{Nguyen2018,
  title = {Towards Quantum Simulation with Circular Rydberg Atoms},
  author = {Nguyen, T. L. and Raimond, J. M. and Sayrin, C. and Corti\~nas, R. and Cantat-Moltrecht, T. and Assemat, F. and Dotsenko, I. and Gleyzes, S. and Haroche, S. and Roux, G. and Jolicoeur, Th. and Brune, M.},
  journal = {Phys. Rev. X},
  volume = {8},
  issue = {1},
  pages = {011032},
  numpages = {27},
  year = {2018},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevX.8.011032},
  url = {https://link.aps.org/doi/10.1103/PhysRevX.8.011032}
}

@article{kuhr2007,
  title={Ultrahigh finesse Fabry-P{\'e}rot superconducting resonator},
  author={Kuhr, Stefan and Gleyzes, S{\'e}bastien and Guerlin, Christine and Bernu, Julien and Hoff, U Busk and Del{\'e}glise, Samuel and Osnaghi, Stefano and Brune, Michel and Raimond, J-M and Haroche, Serge and others},
  journal={Applied Physics Letters},
  volume={90},
  number={16},
  pages={164101},
  year={2007},
  publisher={American Institute of Physics}
}




@article{eickbusch2022,
  title={Fast universal control of an oscillator with weak dispersive coupling to a qubit},
  author={Eickbusch, Alec and Sivak, Volodymyr and Ding, Andy Z and Elder, Salvatore S and Jha, Shantanu R and Venkatraman, Jayameenakshi and Royer, Baptiste and Girvin, SM and Schoelkopf, Robert J and Devoret, Michel H},
  journal={Nature Physics},
  volume={18},
  number={12},
  pages={1464--1469},
  year={2022},
  publisher={Nature Publishing Group UK London}
}

@article{Meinert2020,
  title = {Indium tin oxide films meet circular Rydberg atoms: Prospects for novel quantum simulation schemes},
  author = {Meinert, Florian and H\"olzl, Christian and Nebioglu, Mehmet Ali and D'Arnese, Alessandro and Karl, Philipp and Dressel, Martin and Scheffler, Marc},
  journal = {Phys. Rev. Res.},
  volume = {2},
  issue = {2},
  pages = {023192},
  numpages = {7},
  year = {2020},
  month = {May},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevResearch.2.023192},
  url = {https://link.aps.org/doi/10.1103/PhysRevResearch.2.023192}
}


@article{rondin2017,
  title={Direct measurement of Kramers turnover with a levitated nanoparticle},
  author={Rondin, Lo{\"\i}c and Gieseler, Jan and Ricci, Francesco and Quidant, Romain and Dellago, Christoph and Novotny, Lukas},
  journal={Nature nanotechnology},
  volume={12},
  number={12},
  pages={1130--1133},
  year={2017},
  publisher={Nature Publishing Group UK London}
}

@phdthesis{cortinasPhD2020,
  title={Laser trapping of cold circular Rydberg atoms for quantum simulation},
  author={Corti{\~n}as, Rodrigo Gast{\'o}n},
  year={2020},
  school={{\'E}cole Normale Sup{\'e}rieure (Paris); Paris Sciences et Lettres}
}

@article{Larrouy2020,
  title = {Fast Navigation in a Large Hilbert Space Using Quantum Optimal Control},
  author = {Larrouy, Arthur and Patsch, Sabrina and Richaud, R\'emi and Raimond, Jean-Michel and Brune, Michel and Koch, Christiane P. and Gleyzes, S\'ebastien},
  journal = {Phys. Rev. X},
  volume = {10},
  issue = {2},
  pages = {021058},
  numpages = {14},
  year = {2020},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevX.10.021058},
  url = {https://link.aps.org/doi/10.1103/PhysRevX.10.021058}
}


@article{sautenkov2019,
  title={Optical dipole trap for laser-cooled lithium-7 atoms},
  author={Sautenkov, Vladimir A and Saakyan, Sergey A and Bobrov, Andrey A and Kudrinskiy, Daniil A and Vilshanskaya, Eugenia V and Zelener, Boris B},
  journal={Journal of Russian Laser Research},
  volume={40},
  pages={230--236},
  year={2019},
  publisher={Springer US}
}

@article{Habib1998,
  title = {Decoherence, Chaos, and the Correspondence Principle},
  author = {Habib, Salman and Shizume, Kosuke and Zurek, Wojciech Hubert},
  journal = {Phys. Rev. Lett.},
  volume = {80},
  issue = {20},
  pages = {4361--4365},
  numpages = {0},
  year = {1998},
  month = {May},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.80.4361},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.80.4361}
}


@article{zurek2001,
  title={Sub-Planck structure in phase space and its relevance for quantum decoherence},
  author={Zurek, Wojciech Hubert},
  journal={Nature},
  volume={412},
  number={6848},
  pages={712--717},
  year={2001},
  publisher={Nature Publishing Group}
}




@article{shor1995,
  title = {Scheme for reducing decoherence in quantum computer memory},
  author = {Shor, Peter W.},
  journal = {Phys. Rev. A},
  volume = {52},
  issue = {4},
  pages = {R2493--R2496},
  numpages = {0},
  year = {1995},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.52.R2493},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.52.R2493}
}


@article{chamberland_building_2022,
	title = {Building a {Fault}-{Tolerant} {Quantum} {Computer} {Using} {Concatenated} {Cat} {Codes}},
	volume = {3},
	url = {https://link.aps.org/doi/10.1103/PRXQuantum.3.010329},
	doi = {10.1103/PRXQuantum.3.010329},
	number = {1},
	urldate = {2022-04-29},
	journal = {PRX Quantum},
	author = {Chamberland, Christopher and Noh, Kyungjoo and Arrangoiz-Arriola, Patricio and Campbell, Earl T. and Hann, Connor T. and Iverson, Joseph and Putterman, Harald and Bohdanowicz, Thomas C. and Flammia, Steven T. and Keller, Andrew and Refael, Gil and Preskill, John and Jiang, Liang and Safavi-Naeini, Amir H. and Painter, Oskar and Brandão, Fernando G.S.L.},
	month = feb,
	year = {2022},
	note = {Publisher: American Physical Society},
	pages = {010329},
}

@article{putterman_stabilizing_2022,
	title = {Stabilizing a {Bosonic} {Qubit} {Using} {Colored} {Dissipation}},
	volume = {128},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.128.110502},
	doi = {10.1103/PhysRevLett.128.110502},
	number = {11},
	urldate = {2022-04-29},
	journal = {Physical Review Letters},
	author = {Putterman, Harald and Iverson, Joseph and Xu, Qian and Jiang, Liang and Painter, Oskar and Brandão, Fernando G. S. L. and Noh, Kyungjoo},
	month = mar,
	year = {2022},
	note = {Publisher: American Physical Society},
	pages = {110502},
}

@article{rosenblum2018,
author = {S. Rosenblum  and P. Reinhold  and M. Mirrahimi  and Liang Jiang  and L. Frunzio  and R. J. Schoelkopf },
title = {Fault-tolerant detection of a quantum error},
journal = {Science},
volume = {361},
number = {6399},
pages = {266-270},
year = {2018},
doi = {10.1126/science.aat3996},
URL = {https://www.science.org/doi/abs/10.1126/science.aat3996},
}

@article{roberts2020,
  title = {Driven-Dissipative Quantum Kerr Resonators: New Exact Solutions, Photon Blockade and Quantum Bistability},
  author = {Roberts, David and Clerk, Aashish A.},
  journal = {Phys. Rev. X},
  volume = {10},
  issue = {2},
  pages = {021022},
  numpages = {27},
  year = {2020},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevX.10.021022},
  url = {https://link.aps.org/doi/10.1103/PhysRevX.10.021022}
}

@Unpublished{Burgelman2022,
  doi = {10.48550/ARXIV.2206.14631},
  
  url = {https://arxiv.org/abs/2206.14631},
  
  author = {Burgelman, Michiel and Rouchon, Pierre and Sarlette, Alain and Mirrahimi, Mazyar},
  
  keywords = {Quantum Physics (quant-ph), FOS: Physical sciences, FOS: Physical sciences},
  
  title = {Structurally stable subharmonic regime of a driven quantum Josephson circuit},
  
  year = {2022},
  eprint = {2206.14631},
  archivePrefix = "arXiv",
  primaryClass = "quant-ph",
}







@Article{wwang2019,
author={Wang, W.
and Wu, Y.
and Ma, Y.
and Cai, W.
and Hu, L.
and Mu, X.
and Xu, Y.
and Chen, Zi-Jie
and Wang, H.
and Song, Y. P.
and Yuan, H.
and Zou, C.-L.
and Duan, L.-M.
and Sun, L.},
title={Heisenberg-limited single-mode quantum metrology in a superconducting circuit},
journal={Nature Communications},
year={2019},
month={Sep},
day={26},
volume={10},
number={1},
pages={4382},
abstract={Two-mode interferometers lay the foundations for quantum metrology. Instead of exploring quantum entanglement in the two-mode interferometers, a single bosonic mode also promises a measurement precision beyond the shot-noise limit (SNL) by taking advantage of the infinite-dimensional Hilbert space of Fock states. Here, we demonstrate a single-mode phase estimation that approaches the Heisenberg limit (HL) unconditionally. Due to the strong dispersive nonlinearity and long coherence time of a microwave cavity, quantum states of the form {\$}{\$}{\backslash}left( {\{}{\backslash}left| 0 {\backslash}right{\backslash}rangle + {\backslash}left| N {\backslash}right{\backslash}rangle {\}} {\backslash}right)/{\backslash}sqrt 2{\$}{\$}can be generated, manipulated and detected with high fidelities, leading to an experimental phase estimation precision scaling as ∼N−0.94. A 9.1{\thinspace}dB enhancement of the precision over the SNL at N{\thinspace}={\thinspace}12 is achieved, which is only 1.7{\thinspace}dB away from the HL. Our experimental architecture is hardware efficient and can be combined with quantum error correction techniques to fight against decoherence, and thus promises quantum-enhanced sensing in practical applications.},
issn={2041-1723},
doi={10.1038/s41467-019-12290-7},
url={https://doi.org/10.1038/s41467-019-12290-7}
}


@article{Hatridge2013,
author = {M. Hatridge  and S. Shankar  and M. Mirrahimi  and F. Schackert  and K. Geerlings  and T. Brecht  and K. M. Sliwa  and B. Abdo  and L. Frunzio  and S. M. Girvin  and R. J. Schoelkopf  and M. H. Devoret },
title = {Quantum Back-Action of an Individual Variable-Strength Measurement},
journal = {Science},
volume = {339},
number = {6116},
pages = {178-181},
year = {2013},
doi = {10.1126/science.1226897},
URL = {https://www.science.org/doi/abs/10.1126/science.1226897},
eprint = {https://www.science.org/doi/pdf/10.1126/science.1226897},
abstract = {The actual process of measuring a quantum system has an effect on the result making the outcome unpredictable. Using a superconducting qubit placed in a microwave cavity, Hatridge et al. (p. 178) found that a series of partial measurements on a quantum system left the system in a pure state. Looking at the record of the actual measurements allowed the final state of a superconducting-based quantum system to be determined accurately. Such control is crucial for achieving full feedback control of a general quantum system. The evolution of a quantum system can be tracked via a series of partial measurements that leave the system in a pure state. Measuring a quantum system can randomly perturb its state. The strength and nature of this back-action depend on the quantity that is measured. In a partial measurement performed by an ideal apparatus, quantum physics predicts that the system remains in a pure state whose evolution can be tracked perfectly from the measurement record. We demonstrated this property using a superconducting qubit dispersively coupled to a cavity traversed by a microwave signal. The back-action on the qubit state of a single measurement of both signal quadratures was observed and shown to produce a stochastic operation whose action is determined by the measurement result. This accurate monitoring of a qubit state is an essential prerequisite for measurement-based feedback control of quantum systems.}}


@article{ong2013,
  title = {Quantum Heating of a Nonlinear Resonator Probed by a Superconducting Qubit},
  author = {Ong, F. R. and Boissonneault, M. and Mallet, F. and Doherty, A. C. and Blais, A. and Vion, D. and Esteve, D. and Bertet, P.},
  journal = {Phys. Rev. Lett.},
  volume = {110},
  issue = {4},
  pages = {047001},
  numpages = {5},
  year = {2013},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.110.047001},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.110.047001}
}


@article{ong2011,
  title = {Circuit QED with a Nonlinear Resonator: ac-Stark Shift and Dephasing},
  author = {Ong, F. R. and Boissonneault, M. and Mallet, F. and Palacios-Laloy, A. and Dewes, A. and Doherty, A. C. and Blais, A. and Bertet, P. and Vion, D. and Esteve, D.},
  journal = {Phys. Rev. Lett.},
  volume = {106},
  issue = {16},
  pages = {167002},
  numpages = {4},
  year = {2011},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.106.167002},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.106.167002}
}

@article{girvin2014,
  title={Circuit QED: superconducting qubits coupled to microwave photons},
  author={Girvin, Steven M},
  journal={Quantum machines: measurement and control of engineered quantum systems},
  pages={113--256},
  year={2014},
  publisher={Oxford University Press Oxford}
}

@article{friedman1996,
  title={Macroscopic measurement of resonant magnetization tunneling in high-spin molecules},
  author={Friedman, Jonathan R and Sarachik, MP and Tejada, J and Ziolo, R},
  journal={Physical review letters},
  volume={76},
  number={20},
  pages={3830},
  year={1996},
  publisher={APS}
}


@article{Dykman1975,
author = {Dykman, M. I. and Krivoglaz, M. A.},
title = {Spectral distribution of nonlinear oscillators with nonlinear friction due to a medium},
journal = {physica status solidi (b)},
volume = {68},
number = {1},
pages = {111-123},
doi = {https://doi.org/10.1002/pssb.2220680109},
url = {https://onlinelibrary.wiley.com/doi/abs/10.1002/pssb.2220680109},
abstract = {Abstract The analog of a quantum kinetic equation for the description of time correlation functions of singled out nonlinear oscillators interacting with a medium (e.g. local or quasi-local vibrations in crystals) is obtained. Both the frictions, the linear and nonlinear one (the latter is due to decays with participation of two quanta of singled out oscillators), were taken into account. Spectral distributions of the correlation functions of the coordinates are found as well as those of occupation numbers. The essentially non-Lorentzian shape of the spectral distribution and its dependence on interaction parameters and temperature are analysed.},
year = {1975}
}


@article{Alexander1970,
  title = {Far-Infrared Properties of Lattice Resonant Modes. III. Temperature Effects},
  author = {Alexander, R. W. and Hughes, A. E. and Sievers, A. J.},
  journal = {Phys. Rev. B},
  volume = {1},
  issue = {4},
  pages = {1563--1575},
  numpages = {0},
  year = {1970},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.1.1563},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.1.1563}
  }
  
@article{Merzbacher2002,
author = {Merzbacher,Eugen },
title = {The Early History of Quantum Tunneling},
journal = {Physics Today},
volume = {55},
number = {8},
pages = {44-49},
year = {2002},
doi = {10.1063/1.1510281},
}

@article{gautier_combined_2022,
	title = {Combined {Dissipative} and {Hamiltonian} {Confinement} of {Cat} {Qubits}},
	url = {http://arxiv.org/abs/2112.05545},
	urldate = {2022-03-21},
	journal = {arXiv:2112.05545 [quant-ph]},
	author = {Gautier, Ronan and Sarlette, Alain and Mirrahimi, Mazyar},
	month = feb,
	year = {2022},
	note = {arXiv: 2112.05545},
	keywords = {Quantum Physics},
}

@article{xu_engineering_2022,
	title = {Engineering fast bias-preserving gates on stabilized cat qubits},
	volume = {4},
	url = {https://link.aps.org/doi/10.1103/PhysRevResearch.4.013082},
	doi = {10.1103/PhysRevResearch.4.013082},
	number = {1},
	urldate = {2022-02-09},
	journal = {Physical Review Research},
	author = {Xu, Qian and Iverson, Joseph K. and Brandão, Fernando G. S. L. and Jiang, Liang},
	month = feb,
	year = {2022},
	note = {Publisher: American Physical Society},
	pages = {013082},
}



@article{vijay_invited_2009,
	title = {Invited {Review} {Article}: {The} {Josephson} bifurcation amplifier},
	volume = {80},
	issn = {0034-6748},
	shorttitle = {Invited {Review} {Article}},
	url = {http://aip.scitation.org/doi/10.1063/1.3224703},
	doi = {10.1063/1.3224703},
	number = {11},
	urldate = {2017-02-13},
	journal = {Review of Scientific Instruments},
	author = {Vijay, R. and Devoret, M. H. and Siddiqi, I.},
	month = nov,
	year = {2009},
	pages = {111101},
}


@Article{mazurenko2017,
author={Mazurenko, Anton
and Chiu, Christie S.
and Ji, Geoffrey
and Parsons, Maxwell F.
and Kan{\'a}sz-Nagy, M{\'a}rton
and Schmidt, Richard
and Grusdt, Fabian
and Demler, Eugene
and Greif, Daniel
and Greiner, Markus},
title={A cold-atom Fermi--Hubbard antiferromagnet},
journal={Nature},
year={2017},
month={May},
day={01},
volume={545},
number={7655},
pages={462-466},
abstract={An antiferromagnet with a correlation length that encompasses the whole system is created with the aid of quantum gas microscopy of cold atoms in an optical lattice.},
issn={1476-4687},
doi={10.1038/nature22362},
url={https://doi.org/10.1038/nature22362}
}

@Article{Bakr2009,
author={Bakr, Waseem S.
and Gillen, Jonathon I.
and Peng, Amy
and F{\"o}lling, Simon
and Greiner, Markus},
title={A quantum gas microscope for detecting single atoms in a Hubbard-regime optical lattice},
journal={Nature},
year={2009},
month={Nov},
day={01},
volume={462},
number={7269},
pages={74-77},
abstract={A new quantum gas microscope that bridges the gap between microscopic and macroscopic approaches to the study of quantum systems has been developed. It uses high-resolution optical imaging to detect single atoms held in a holographically generated optical lattice. Its potential is demonstrated by the production of images of single rubidium atoms confined to an optical lattice with spacings of just 640 nanometres between atoms. The approach should facilitate quantum simulation of condensed-matter systems and find possible application in addressing and read-out of large-scale quantum information systems based on ultracold atoms.},
issn={1476-4687},
doi={10.1038/nature08482},
url={https://doi.org/10.1038/nature08482}
}

@Article{Slocombe2022,
author={Slocombe, Louie
and Sacchi, Marco
and Al-Khalili, Jim},
title={An open quantum systems approach to proton tunnelling in DNA},
journal={Communications Physics},
year={2022},
month={May},
day={05},
volume={5},
number={1},
pages={109},
abstract={One of the most important topics in molecular biology is the genetic stability of DNA. One threat to this stability is proton transfer along the hydrogen bonds of DNA that could lead to tautomerisation, hence creating point mutations. We present a theoretical analysis of the hydrogen bonds between the Guanine-Cytosine (G-C) nucleotide, which includes an accurate model of the structure of the base pairs, the quantum dynamics of the hydrogen bond proton, and the influence of the decoherent and dissipative cellular environment. We determine that the quantum tunnelling contribution to the proton transfer rate is several orders of magnitude larger than the classical over-the-barrier hopping. Due to the significance of the quantum tunnelling even at biological temperatures, we find that the canonical and tautomeric forms of G-C inter-convert over timescales far shorter than biological ones and hence thermal equilibrium is rapidly reached. Furthermore, we find a large tautomeric occupation probability of 1.73{\thinspace}{\texttimes}{\thinspace}10−4, suggesting that such proton transfer may well play a far more important role in DNA mutation than has hitherto been suggested. Our results could have far-reaching consequences for current models of genetic mutations.},
issn={2399-3650},
doi={10.1038/s42005-022-00881-8},
url={https://doi.org/10.1038/s42005-022-00881-8}
}


@Article{Krantz2016,
author={Krantz, Philip
and Bengtsson, Andreas
and Simoen, Micha{\"e}l
and Gustavsson, Simon
and Shumeiko, Vitaly
and Oliver, W. D.
and Wilson, C. M.
and Delsing, Per
and Bylander, Jonas},
title={Single-shot read-out of a superconducting qubit using a Josephson parametric oscillator},
journal={Nature Communications},
year={2016},
month={May},
day={09},
volume={7},
number={1},
pages={11417},
abstract={We propose and demonstrate a read-out technique for a superconducting qubit by dispersively coupling it with a Josephson parametric oscillator. We employ a tunable quarter wavelength superconducting resonator and modulate its resonant frequency at twice its value with an amplitude surpassing the threshold for parametric instability. We map the qubit states onto two distinct states of classical parametric oscillation: one oscillating state, with 185{\textpm}15 photons in the resonator, and one with zero oscillation amplitude. This high contrast obviates a following quantum-limited amplifier. We demonstrate proof-of-principle, single-shot read-out performance, and present an error budget indicating that this method can surpass the fidelity threshold required for quantum computing.},
issn={2041-1723},
doi={10.1038/ncomms11417},
url={https://doi.org/10.1038/ncomms11417}
}





@article{Wustmann2013,
  title = {Parametric resonance in tunable superconducting cavities},
  author = {Wustmann, Waltraut and Shumeiko, Vitaly},
  journal = {Phys. Rev. B},
  volume = {87},
  issue = {18},
  pages = {184501},
  numpages = {23},
  year = {2013},
  month = {May},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.87.184501},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.87.184501}
}


@article{Wustmann2019,
author = {Wustmann,Waltraut  and Shumeiko,Vitaly },
title = {Parametric effects in circuit quantum electrodynamics},
journal = {Low Temperature Physics},
volume = {45},
number = {8},
pages = {848-869},
year = {2019},
doi = {10.1063/1.5116533},

URL = { 
        https://doi.org/10.1063/1.5116533
    
},

}

@article{Carusotto2013,
  title = {Quantum fluids of light},
  author = {Carusotto, Iacopo and Ciuti, Cristiano},
  journal = {Rev. Mod. Phys.},
  volume = {85},
  issue = {1},
  pages = {299--366},
  numpages = {0},
  year = {2013},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/RevModPhys.85.299},
  url = {https://link.aps.org/doi/10.1103/RevModPhys.85.299}
}

@article{condensed, title={Photonic materials in circuit quantum electrodynamics}, volume={16}, url={http://dx.doi.org/10.1038/s41567-020-0815-y}, DOI={10.1038/s41567-020-0815-y}, number={3}, journal={Nature Physics}, publisher={Springer Science and Business Media LLC}, author={Carusotto, Iacopo and Houck, Andrew A. and Kollár, Alicia J. and Roushan, Pedram and Schuster, David I. and Simon, Jonathan}, year={2020}, month=mar, pages={268–279}, language={english} }

@article{minganti2016,
  title={Exact results for Schr{\"o}dinger cats in driven-dissipative systems and their feedback control},
  author={Minganti, Fabrizio and Bartolo, Nicola and Lolli, Jared and Casteels, Wim and Ciuti, Cristiano},
  journal={Scientific reports},
  volume={6},
  number={1},
  pages={1--8},
  year={2016},
  publisher={Nature Publishing Group}
}




@article{Slobodskyy2003,
  title = {Voltage-Controlled Spin Selection in a Magnetic Resonant Tunneling Diode},
  author = {Slobodskyy, A. and Gould, C. and Slobodskyy, T. and Becker, C. R. and Schmidt, G. and Molenkamp, L. W.},
  journal = {Phys. Rev. Lett.},
  volume = {90},
  issue = {24},
  pages = {246601},
  numpages = {4},
  year = {2003},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.90.246601},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.90.246601}
}

@article{SM,
note = {See Supplemental Material at [url] }
}


@article{Joyez1997,
  title = {Strong Tunneling in the Single-Electron Transistor},
  author = {Joyez, P. and Bouchiat, V. and Esteve, D. and Urbina, C. and Devoret, M. H.},
  journal = {Phys. Rev. Lett.},
  volume = {79},
  issue = {7},
  pages = {1349--1352},
  numpages = {0},
  year = {1997},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.79.1349},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.79.1349}
}

@article{fosco2013,
  title = {Vacuum fluctuations and generalized boundary conditions},
  author = {Fosco, César D. and Lombardo, Fernando C. and  Mazzitelli, Francisco D.},
  journal = {Phys. Rev. D},
  volume = {87},
  issue = {10},
  pages = {105008},
  numpages = {0},
  year = {2013},
  month = {May},
  publisher = {American Physical Society},
  doi = {https://doi.org/10.1103/PhysRevD.87.105008},
  url = {https://journals.aps.org/prd/abstract/10.1103/PhysRevD.87.105008}
}

@article{Spielmann1994,
  title = {Tunneling of Optical Pulses through Photonic Band Gaps},
  author = {Spielmann, Ch. and Szip\"ocs, R. and Stingl, A. and Krausz, F.},
  journal = {Phys. Rev. Lett.},
  volume = {73},
  issue = {17},
  pages = {2308--2311},
  numpages = {0},
  year = {1994},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.73.2308},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.73.2308}
}


@article{Steinberg1993,
  title = {Measurement of the single-photon tunneling time},
  author = {Steinberg, A. M. and Kwiat, P. G. and Chiao, R. Y.},
  journal = {Phys. Rev. Lett.},
  volume = {71},
  issue = {5},
  pages = {708--711},
  numpages = {0},
  year = {1993},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.71.708},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.71.708}
}


@Article{DEVAULT1967,
author={DeVault, Don
and Parkes, John H.
and Chance, Britton},
title={Electron Tunnelling in Cytochromes},
journal={Nature},
year={1967},
month={Aug},
day={01},
volume={215},
number={5101},
pages={642-644},
abstract={OXIDATION of a c-type cytochrome by light absorbed by the photosynthetic system of the purple sulphur bacterium, Chromatium, at the temperature of liquid nitrogen was discovered by Chance and Nishimura1. Vredenberg and Duysens2 made further measurements confirming that quantum efficiencies did not change by more than a factor of two, if that much, at the lowest temperatures. The light and instrument limitations on these measurements make any further conclusions about rates difficult.},
issn={1476-4687},
doi={10.1038/215642a0},
url={https://doi.org/10.1038/215642a0}
}



@article{Kolesnikov2016,
  title = {Quantum Tunneling of Water in Beryl: A New State of the Water Molecule},
  author = {Kolesnikov, Alexander I. and Reiter, George F. and Choudhury, Narayani and Prisk, Timothy R. and Mamontov, Eugene and Podlesnyak, Andrey and Ehlers, George and Seel, Andrew G. and Wesolowski, David J. and Anovitz, Lawrence M.},
  journal = {Phys. Rev. Lett.},
  volume = {116},
  issue = {16},
  pages = {167802},
  numpages = {6},
  year = {2016},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.116.167802},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.116.167802}
}



@article{aidelsburger2013,
  title = {Realization of the Hofstadter Hamiltonian with Ultracold Atoms in Optical Lattices},
  author = {Aidelsburger, M. and Atala, M. and Lohse, M. and Barreiro, J. T. and Paredes, B. and Bloch, I.},
  journal = {Phys. Rev. Lett.},
  volume = {111},
  issue = {18},
  pages = {185301},
  numpages = {5},
  year = {2013},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.111.185301},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.111.185301}
}


@Article{Schafer2020,
author={Sch{\"a}fer, Florian
and Fukuhara, Takeshi
and Sugawa, Seiji
and Takasu, Yosuke
and Takahashi, Yoshiro},
title={Tools for quantum simulation with ultracold atoms in optical lattices},
journal={Nature Reviews Physics},
year={2020},
month={Aug},
day={01},
volume={2},
number={8},
pages={411-425},
abstract={After many years of development of the basic tools, quantum simulation with ultracold atoms has now reached the level of maturity at which it can be used to investigate complex quantum processes. Planning of new experiments and upgrading of existing set-ups requires a broad overview of the available techniques, their specific advantages and limitations. This Technical Review aims to provide a comprehensive compendium of the state of the art. We discuss the basic principles, the available techniques and their current range of applications. Focusing on the simulation of various phenomena in solid-state physics through optical lattice experiments, we review their basics, the necessary techniques and the accessible physical parameters. We outline how to control and use interactions with external potentials and interactions between the atoms, and how to design new synthetic gauge fields and spin--orbit coupling. We discuss the latest progress in site-resolved techniques that use quantum gas microscopes, and describe the unique features of quantum simulation experiments with two-electron atomic species.},
issn={2522-5820},
doi={10.1038/s42254-020-0195-3},
url={https://doi.org/10.1038/s42254-020-0195-3}
}

@Article{Bloch2012,
author={Bloch, Immanuel
and Dalibard, Jean
and Nascimb{\`e}ne, Sylvain},
title={Quantum simulations with ultracold quantum gases},
journal={Nature Physics},
year={2012},
month={Apr},
day={01},
volume={8},
number={4},
pages={267-276},
abstract={Ultracold quantum gases offer a unique setting for quantum simulation of interacting many-body systems. The high degree of controllability, the novel detection possibilities and the extreme physical parameter regimes that can be reached in these `artificial solids' provide an exciting complementary set-up compared with natural condensed-matter systems, much in the spirit of Feynman's vision of a quantum simulator. Here we review recent advances in technology and discuss progress in a number of areas where experimental results have already been obtained.},
issn={1745-2481},
doi={10.1038/nphys2259},
url={https://doi.org/10.1038/nphys2259}
}

@article{kaufman2014,
  title={Two-particle quantum interference in tunnel-coupled optical tweezers},
  author={Kaufman, AM and Lester, BJ and Reynolds, CM and Wall, ML and Foss-Feig, M and Hazzard, KRA and Rey, AM and Regal, CA},
  journal={Science},
  volume={345},
  number={6194},
  pages={306--309},
  year={2014},
  publisher={American Association for the Advancement of Science}
}
@article{noguchi2014,
  title={Aharonov--Bohm effect in the tunnelling of a quantum rotor in a linear Paul trap},
  author={Noguchi, Atsushi and Shikano, Yutaka and Toyoda, Kenji and Urabe, Shinji},
  journal={Nature communications},
  volume={5},
  number={1},
  pages={1--6},
  year={2014},
  publisher={Nature Publishing Group}
}

@article{kierig2008,
  title={Single-particle tunneling in strongly driven double-well potentials},
  author={Kierig, E and Schnorrberger, U and Schietinger, A and Tomkovic, J and Oberthaler, MK},
  journal={Physical review letters},
  volume={100},
  number={19},
  pages={190405},
  year={2008},
  publisher={APS}
}

@article{ma2011,
  title={Photon-assisted tunneling in a biased strongly correlated Bose gas},
  author={Ma, Ruichao and Tai, M Eric and Preiss, Philipp M and Bakr, Waseem S and Simon, Jonathan and Greiner, Markus},
  journal={Physical Review Letters},
  volume={107},
  number={9},
  pages={095301},
  year={2011},
  publisher={APS}
}


@article{folling2007,
  title={Direct observation of second-order atom tunnelling},
  author={F{\"o}lling, Simon and Trotzky, Stefan and Cheinet, Patrick and Feld, Michael and Saers, Robert and Widera, Artur and M{\"u}ller, Torben and Bloch, Immanuel},
  journal={Nature},
  volume={448},
  number={7157},
  pages={1029--1032},
  year={2007},
  publisher={Nature Publishing Group}
}

@article{ramos2020,
  title={Measurement of the time spent by a tunnelling atom within the barrier region},
  author={Ramos, Ram{\'o}n and Spierings, David and Racicot, Isabelle and Steinberg, Aephraim M},
  journal={Nature},
  volume={583},
  number={7817},
  pages={529--532},
  year={2020},
  publisher={Nature Publishing Group}
}


@article{nakamura_coherent_1999,
	title = {Coherent control of macroscopic quantum states in a single-{Cooper}-pair box},
	volume = {398},
	copyright = {1999 Macmillan Magazines Ltd.},
	issn = {1476-4687},
	url = {https://www.nature.com/articles/19718},
	doi = {10.1038/19718},
	language = {english},
	number = {6730},
	urldate = {2022-05-10},
	journal = {Nature},
	author = {Nakamura, Y. and Pashkin, Yu A. and Tsai, J. S.},
	month = apr,
	year = {1999},
	note = {Number: 6730
Publisher: Nature Publishing Group},
	keywords = {Humanities and Social Sciences, multidisciplinary, Science},
	pages = {786--788},
}

@article{lescanne_escape_2019,
	title = {Escape of a {Driven} {Quantum} {Josephson} {Circuit} into {Unconfined} {States}},
	volume = {11},
	url = {https://link.aps.org/doi/10.1103/PhysRevApplied.11.014030},
	doi = {10.1103/PhysRevApplied.11.014030},
	number = {1},
	urldate = {2021-06-18},
	journal = {Physical Review Applied},
	author = {Lescanne, Raphaël and Verney, Lucas and Ficheux, Quentin and Devoret, Michel H. and Huard, Benjamin and Mirrahimi, Mazyar and Leghtas, Zaki},
	month = jan,
	year = {2019},
	note = {Publisher: American Physical Society},
	pages = {014030},
}

@article{guo_phase_2013,
	title = {Phase {Space} {Crystals}: {A} {New} {Way} to {Create} a {Quasienergy} {Band} {Structure}},
	volume = {111},
	shorttitle = {Phase {Space} {Crystals}},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.111.205303},
	doi = {10.1103/PhysRevLett.111.205303},
	number = {20},
	urldate = {2022-05-10},
	journal = {Physical Review Letters},
	author = {Guo, Lingzhen and Marthaler, Michael and Schön, Gerd},
	month = nov,
	year = {2013},
	note = {Publisher: American Physical Society},
	pages = {205303},
}

@article{svensson_period_2018,
	title = {Period multiplication in a parametrically driven superconducting resonator},
	volume = {113},
	issn = {0003-6951},
	url = {https://aip.scitation.org/doi/full/10.1063/1.5026974},
	doi = {10.1063/1.5026974},
	number = {2},
	urldate = {2021-07-27},
	journal = {Applied Physics Letters},
	author = {Svensson, Ida-Maria and Bengtsson, Andreas and Bylander, Jonas and Shumeiko, Vitaly and Delsing, Per},
	month = jul,
	year = {2018},
	note = {Publisher: American Institute of Physics},
	pages = {022602},
}

@article{wilson, title={Observation of the dynamical Casimir effect in a superconducting circuit}, volume={479}, url={http://dx.doi.org/10.1038/nature10561}, DOI={10.1038/nature10561}, number={7373}, journal={Nature}, publisher={Springer Science and Business Media LLC}, author={Wilson, C. M. and Johansson, G. and Pourkabirian, A. and Simoen, M. and Johansson, J. R. and Duty, T. and Nori, F. and Delsing, P.}, year={2011}, month=nov, pages={376–379}, language={english} }

@article{paraoanu,
author = {Pasi Lähteenmäki  and G. S. Paraoanu  and Juha Hassel  and Pertti J. Hakonen },
title = {Dynamical Casimir effect in a Josephson metamaterial},
journal = {Proceedings of the National Academy of Sciences},
volume = {110},
number = {11},
pages = {4234-4238},
year = {2013},
doi = {10.1073/pnas.1212705110},
URL = {https://www.pnas.org/doi/abs/10.1073/pnas.1212705110},
eprint = {https://www.pnas.org/doi/pdf/10.1073/pnas.1212705110},
abstract = {The zero-point energy stored in the modes of an electromagnetic cavity has experimentally detectable effects, giving rise to an attractive interaction between the opposite walls, the static Casimir effect. A dynamical version of this effect was predicted to occur when the vacuum energy is changed either by moving the walls of the cavity or by changing the index of refraction, resulting in the conversion of vacuum fluctuations into real photons. Here, we demonstrate the dynamical Casimir effect using a Josephson metamaterial embedded in a microwave cavity at 5.4 GHz. We modulate the effective length of the cavity by flux-biasing the metamaterial based on superconducting quantum interference devices (SQUIDs), which results in variation of a few percentage points in the speed of light. We extract the full 4 × 4 covariance matrix of the emitted microwave radiation, demonstrating that photons at frequencies symmetrical with respect to half of the modulation frequency are generated in pairs. At large detunings of the cavity from half of the modulation frequency, we find power spectra that clearly show the theoretically predicted hallmark of the Casimir effect: a bimodal, “sparrow-tail” structure. The observed substantial photon flux cannot be assigned to parametric amplification of thermal fluctuations; its creation is a direct consequence of the noncommutativity structure of quantum field theory.}}

@article{krantz_single-shot_2016,
	title = {Single-shot read-out of a superconducting qubit using a {Josephson} parametric oscillator},
	volume = {7},
	copyright = {2016 Nature Publishing Group},
	issn = {2041-1723},
	url = {https://www.nature.com/articles/ncomms11417},
	doi = {10.1038/ncomms11417},
	language = {english},
	urldate = {2017-08-16},
	journal = {Nature Communications},
	author = {Krantz, Philip and Bengtsson, Andreas and Simoen, Michaël and Gustavsson, Simon and Shumeiko, Vitaly and Oliver, W. D. and Wilson, C. M. and Delsing, Per and Bylander, Jonas},
	month = may,
	year = {2016},
	pages = {ncomms11417},
}

@article{rosenthal_efficient_2021,
	title = {Efficient and {Low}-{Backaction} {Quantum} {Measurement} {Using} a {Chip}-{Scale} {Detector}},
	volume = {126},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.126.090503},
	doi = {10.1103/PhysRevLett.126.090503},
	number = {9},
	urldate = {2022-05-11},
	journal = {Physical Review Letters},
	author = {Rosenthal, Eric I. and Schneider, Christian M. F. and Malnou, Maxime and Zhao, Ziyi and Leditzky, Felix and Chapman, Benjamin J. and Wustmann, Waltraut and Ma, Xizheng and Palken, Daniel A. and Zanner, Maximilian F. and Vale, Leila R. and Hilton, Gene C. and Gao, Jiansong and Smith, Graeme and Kirchmair, Gerhard and Lehnert, K. W.},
	month = mar,
	year = {2021},
	note = {Publisher: American Physical Society},
	pages = {090503},
}

@article{berdou_one_2022,
	title = {One hundred second bit-flip time in a two-photon dissipative oscillator},
	url = {http://arxiv.org/abs/2204.09128},
	urldate = {2022-05-11},
	journal = {arXiv:2204.09128 [quant-ph]},
	author = {Berdou, C. and Murani, A. and Reglade, U. and Smith, W. C. and Villiers, M. and Palomo, J. and Rosticher, M. and Denis, A. and Morfin, P. and Delbecq, M. and Kontos, T. and Pankratova, N. and Rautschke, F. and Peronnin, T. and Sellem, L.-A. and Rouchon, P. and Sarlette, A. and Mirrahimi, M. and Campagne-Ibarcq, P. and Jezouin, S. and Lescanne, R. and Leghtas, Z.},
	month = apr,
	year = {2022},
	note = {arXiv: 2204.09128},
	keywords = {Quantum Physics},
}

@article{didier_fast_2015,
	title = {Fast {Quantum} {Nondemolition} {Readout} by {Parametric} {Modulation} of {Longitudinal} {Qubit}-{Oscillator} {Interaction}},
	volume = {115},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.115.203601},
	doi = {10.1103/PhysRevLett.115.203601},
	number = {20},
	urldate = {2020-05-08},
	journal = {Physical Review Letters},
	author = {Didier, Nicolas and Bourassa, Jérôme and Blais, Alexandre},
	month = nov,
	year = {2015},
	note = {Publisher: American Physical Society},
	pages = {203601},
}

@article{campagne-ibarcq_observing_2016,
	title = {Observing {Quantum} {State} {Diffusion} by {Heterodyne} {Detection} of {Fluorescence}},
	volume = {6},
	url = {https://link.aps.org/doi/10.1103/PhysRevX.6.011002},
	doi = {10.1103/PhysRevX.6.011002},
	number = {1},
	journal = {Physical Review X},
	author = {Campagne-Ibarcq, P. and Six, P. and Bretheau, L. and Sarlette, A. and Mirrahimi, M. and Rouchon, P. and Huard, B.},
	month = jan,
	year = {2016},
	pages = {011002},
}

@article{pfaff_controlled_2017,
	title = {Controlled release of multiphoton quantum states from a microwave cavity memory},
	volume = {13},
	copyright = {2017 Nature Publishing Group},
	issn = {1745-2481},
	url = {https://www.nature.com/articles/nphys4143},
	doi = {10.1038/nphys4143},
	language = {english},
	number = {9},
	urldate = {2018-05-15},
	journal = {Nature Physics},
	author = {Pfaff, Wolfgang and Axline, Christopher J. and Burkhart, Luke D. and Vool, Uri and Reinhold, Philip and Frunzio, Luigi and Jiang, Liang and Devoret, Michel H. and Schoelkopf, Robert J.},
	month = sep,
	year = {2017},
	pages = {882--887},
}

@article{frattini_optimizing_2018,
	title = {Optimizing the {Nonlinearity} and {Dissipation} of a {SNAIL} {Parametric} {Amplifier} for {Dynamic} {Range}},
	volume = {10},
	url = {https://link.aps.org/doi/10.1103/PhysRevApplied.10.054020},
	doi = {10.1103/PhysRevApplied.10.054020},
	number = {5},
	journal = {Physical Review Applied},
	author = {Frattini, N. E. and Sivak, V. V. and Lingenfelter, A. and Shankar, S. and Devoret, M. H.},
	month = nov,
	year = {2018},
	pages = {054020},
}

@article{sivak_kerr-free_2019,
	title = {Kerr-{Free} {Three}-{Wave} {Mixing} in {Superconducting} {Quantum} {Circuits}},
	volume = {11},
	url = {https://link.aps.org/doi/10.1103/PhysRevApplied.11.054060},
	doi = {10.1103/PhysRevApplied.11.054060},
	number = {5},
	journal = {Physical Review Applied},
	author = {Sivak, V.V. and Frattini, N.E. and Joshi, V.R. and Lingenfelter, A. and Shankar, S. and Devoret, M.H.},
	month = may,
	year = {2019},
	pages = {054060},
}

@article{axline_architecture_2016,
	title = {An architecture for integrating planar and {3D} {cQED} devices},
	volume = {109},
	issn = {0003-6951},
	url = {https://aip.scitation.org/doi/10.1063/1.4959241},
	doi = {10.1063/1.4959241},
	number = {4},
	urldate = {2019-10-07},
	journal = {Applied Physics Letters},
	author = {Axline, C. and Reagor, M. and Heeres, R. and Reinhold, P. and Wang, C. and Shain, K. and Pfaff, W. and Chu, Y. and Frunzio, L. and Schoelkopf, R. J.},
	month = jul,
	year = {2016},
	pages = {042601},
}

@article{nigg_black-box_2012,
	title = {Black-{Box} {Superconducting} {Circuit} {Quantization}},
	volume = {108},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.108.240502},
	doi = {10.1103/PhysRevLett.108.240502},
	number = {24},
	journal = {Physical Review Letters},
	author = {Nigg, Simon E. and Paik, Hanhee and Vlastakis, Brian and Kirchmair, Gerhard and Shankar, S. and Frunzio, Luigi and Devoret, M. H. and Schoelkopf, R. J. and Girvin, S. M.},
	month = jun,
	year = {2012},
	pages = {240502},
}

@article{minev_energy-participation_2021,
	title = {Energy-participation quantization of {Josephson} circuits},
	url = {http://arxiv.org/abs/2010.00620},
	urldate = {2021-08-19},
	journal = {arXiv:2010.00620 [cond-mat, physics:quant-ph]},
	author = {Minev, Zlatko K. and Leghtas, Zaki and Mundhada, Shantanu O. and Christakis, Lysander and Pop, Ioan M. and Devoret, Michel H.},
	month = aug,
	year = {2021},
	note = {arXiv: 2010.00620},
	keywords = {Condensed Matter - Superconductivity, Quantum Physics},
}

@article{chow_simple_2011,
	title = {Simple {All}-{Microwave} {Entangling} {Gate} for {Fixed}-{Frequency} {Superconducting} {Qubits}},
	volume = {107},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.107.080502},
	doi = {10.1103/PhysRevLett.107.080502},
	number = {8},
	urldate = {2022-06-08},
	journal = {Physical Review Letters},
	author = {Chow, Jerry M. and Córcoles, A. D. and Gambetta, Jay M. and Rigetti, Chad and Johnson, B. R. and Smolin, John A. and Rozen, J. R. and Keefe, George A. and Rothwell, Mary B. and Ketchen, Mark B. and Steffen, M.},
	month = aug,
	year = {2011},
	note = {Publisher: American Physical Society},
	pages = {080502},
}

@article{castellanos-beltran_amplification_2008,
	title = {Amplification and squeezing of quantum noise with a tunable {Josephson} metamaterial},
	volume = {4},
	copyright = {© 2008 Nature Publishing Group},
	issn = {1745-2473},
	url = {http://www.nature.com/nphys/journal/v4/n12/full/nphys1090.html},
	doi = {10.1038/nphys1090},
	language = {english},
	number = {12},
	urldate = {2016-08-22},
	journal = {Nature Physics},
	author = {Castellanos-Beltran, M. A. and Irwin, K. D. and Hilton, G. C. and Vale, L. R. and Lehnert, K. W.},
	month = dec,
	year = {2008},
	pages = {929--931},
}

@article{muppalla_bistability_2018,
	title = {Bistability in a mesoscopic {Josephson} junction array resonator},
	volume = {97},
	url = {https://link.aps.org/doi/10.1103/PhysRevB.97.024518},
	doi = {10.1103/PhysRevB.97.024518},
	number = {2},
	journal = {Physical Review B},
	author = {Muppalla, P. R. and Gargiulo, O. and Mirzaei, S. I. and Venkatesh, B. Prasanna and Juan, M. L. and Grünhaupt, L. and Pop, I. M. and Kirchmair, G.},
	month = jan,
	year = {2018},
	pages = {024518},
}

@article{turlot_escape_1989,
	title = {Escape oscillations of a {Josephson} junction switching out of the zero-voltage state},
	volume = {62},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.62.1788},
	doi = {10.1103/PhysRevLett.62.1788},
	number = {15},
	urldate = {2022-06-09},
	journal = {Physical Review Letters},
	author = {Turlot, Emmanuel and Esteve, Daniel and Urbina, Cristian and Martinis, John M. and Devoret, Michel H. and Linkwitz, Sebastian and Grabert, Hermann},
	month = apr,
	year = {1989},
	note = {Publisher: American Physical Society},
	pages = {1788--1791},
}

@article{silvestrini_effect_1988,
	title = {Effect of dissipation on thermal activation in an underdamped {Josephson} junction: {First} evidence of a transition between different damping regimes},
	volume = {60},
	shorttitle = {Effect of dissipation on thermal activation in an underdamped {Josephson} junction},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.60.844},
	doi = {10.1103/PhysRevLett.60.844},
	number = {9},
	urldate = {2022-06-09},
	journal = {Physical Review Letters},
	author = {Silvestrini, Paolo and Pagano, Sergio and Cristiano, Roberto and Liengme, O. and Gray, K. E.},
	month = feb,
	year = {1988},
	note = {Publisher: American Physical Society},
	pages = {844--847},
}

@article{wilson_photon_2010,
	title = {Photon {Generation} in an {Electromagnetic} {Cavity} with a {Time}-{Dependent} {Boundary}},
	volume = {105},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.105.233907},
	doi = {10.1103/PhysRevLett.105.233907},
	number = {23},
	urldate = {2022-06-09},
	journal = {Physical Review Letters},
	author = {Wilson, C. M. and Duty, T. and Sandberg, M. and Persson, F. and Shumeiko, V. and Delsing, P.},
	month = dec,
	year = {2010},
	note = {Publisher: American Physical Society},
	pages = {233907},
}

@article{paik_experimental_2016,
	title = {Experimental {Demonstration} of a {Resonator}-{Induced} {Phase} {Gate} in a {Multiqubit} {Circuit}-{QED} {System}},
	volume = {117},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.117.250502},
	doi = {10.1103/PhysRevLett.117.250502},
	number = {25},
	urldate = {2022-06-09},
	journal = {Physical Review Letters},
	author = {Paik, Hanhee and Mezzacapo, A. and Sandberg, Martin and McClure, D. T. and Abdo, B. and Córcoles, A. D. and Dial, O. and Bogorin, D. F. and Plourde, B. L. T. and Steffen, M. and Cross, A. W. and Gambetta, J. M. and Chow, Jerry M.},
	month = dec,
	year = {2016},
	note = {Publisher: American Physical Society},
	pages = {250502},
}

@article{Deleglise_2008, title={Reconstruction of non-classical cavity field states with snapshots of their decoherence}, volume={455}, url={http://dx.doi.org/10.1038/nature07288}, DOI={10.1038/nature07288}, number={7212}, journal={Nature}, publisher={Springer Science and Business Media LLC}, author={Deléglise, Samuel and Dotsenko, Igor and Sayrin, Clément and Bernu, Julien and Brune, Michel and Raimond, Jean-Michel and Haroche, Serge}, year={2008}, month=sep, pages={510–514}, language={en} }

@article{Google_2022, title={Suppressing quantum errors by scaling a surface code logical qubit}, author={Google Quantum AI}, volume={614}, url={http://dx.doi.org/10.1038/s41586-022-05434-1}, DOI={10.1038/s41586-022-05434-1}, number={7949}, journal={Nature}, publisher={Springer Science and Business Media LLC},  year={2023}, month=feb, pages={676–681}, language={en} }

@article{Krinner_2022, title={Realizing repeated quantum error correction in a distance-three surface code}, volume={605}, url={http://dx.doi.org/10.1038/s41586-022-04566-8}, DOI={10.1038/s41586-022-04566-8}, number={7911}, journal={Nature}, publisher={Springer Science and Business Media LLC}, author={Krinner, Sebastian and Lacroix, Nathan and Remm, Ants and Di Paolo, Agustin and Genois, Elie and Leroux, Catherine and Hellings, Christoph and Lazar, Stefania and Swiadek, Francois and Herrmann, Johannes and Norris, Graham J. and Andersen, Christian Kraglund and Müller, Markus and Blais, Alexandre and Eichler, Christopher and Wallraff, Andreas}, year={2022}, month=may, pages={669–674}, language={en} }



@article{monroe1996,
  title={A “Schr{\"o}dinger cat” superposition state of an atom},
  author={Monroe, Christopher and Meekhof, Dawn M and King, Brian E and Wineland, David J},
  journal={Science},
  volume={272},
  number={5265},
  pages={1131--1136},
  year={1996},
  publisher={American Association for the Advancement of Science}
}

@article{hu2019,
  title={Quantum error correction and universal gate set operation on a binomial bosonic logical qubit},
  author={Hu, Ling and Ma, Yuwei and Cai, Weizhou and Mu, Xianghao and Xu, Yuan and Wang, Weiting and Wu, Yukai and Wang, Haiyan and Song, YP and Zou, C-L and others},
  journal={Nature Physics},
  volume={15},
  number={5},
  pages={503--508},
  year={2019},
  publisher={Nature Publishing Group UK London}
}

@article{aspect1982,
  title={Experimental realization of Einstein-Podolsky-Rosen-Bohm Gedankenexperiment: a new violation of Bell's inequalities},
  author={Aspect, Alain and Grangier, Philippe and Roger, G{\'e}rard},
  journal={Physical review letters},
  volume={49},
  number={2},
  pages={91},
  year={1982},
  publisher={APS}
}

@article{Ketterle2002,
  title = {Nobel lecture: When atoms behave as waves: Bose-Einstein condensation and the atom laser},
  author = {Ketterle, Wolfgang},
  journal = {Rev. Mod. Phys.},
  volume = {74},
  issue = {4},
  pages = {1131--1151},
  numpages = {0},
  year = {2002},
  month = {Nov},
  publisher = {American Physical Society},
  doi = {10.1103/RevModPhys.74.1131},
  url = {https://link.aps.org/doi/10.1103/RevModPhys.74.1131}
}


@article{kastler1957,
  title={Optical methods of atomic orientation and of magnetic resonance},
  author={Kastler, Alfred},
  journal={JOSA},
  volume={47},
  number={6},
  pages={460--465},
  year={1957},
  publisher={Optica Publishing Group}
}
@misc{Teoh2022,
  doi = {10.48550/ARXIV.2212.12077},
  
  url = {https://arxiv.org/abs/2212.12077},
  
  author = {Teoh, James D. and Winkel, Patrick and Babla, Harshvardhan K. and Chapman, Benjamin J. and Claes, Jahan and de Graaf, Stijn J. and Garmon, John W. O. and Kalfus, William D. and Lu, Yao and Maiti, Aniket and Sahay, Kaavya and Thakur, Neel and Tsunoda, Takahiro and Xue, Sophia H. and Frunzio, Luigi and Girvin, Steven M. and Puri, Shruti and Schoelkopf, Robert J.},
  
  keywords = {Quantum Physics (quant-ph), FOS: Physical sciences, FOS: Physical sciences},
  
  title = {Dual-rail encoding with superconducting cavities},
  
  publisher = {arXiv},
  
  year = {2022},
  
  copyright = {Creative Commons Attribution Non Commercial Share Alike 4.0 International}
}


@article{Michael2016,
  title = {New Class of Quantum Error-Correcting Codes for a Bosonic Mode},
  author = {Michael, Marios H. and Silveri, Matti and Brierley, R. T. and Albert, Victor V. and Salmilehto, Juha and Jiang, Liang and Girvin, S. M.},
  journal = {Phys. Rev. X},
  volume = {6},
  issue = {3},
  pages = {031006},
  numpages = {26},
  year = {2016},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevX.6.031006},
  url = {https://link.aps.org/doi/10.1103/PhysRevX.6.031006}
}


@article{grimsmo_quantum_2021,
	title = {Quantum {Error} {Correction} with the {Gottesman}-{Kitaev}-{Preskill} {Code}},
	volume = {2},
	url = {https://link.aps.org/doi/10.1103/PRXQuantum.2.020101},
	doi = {10.1103/PRXQuantum.2.020101},
	abstract = {The Gottesman-Kitaev-Preskill (GKP) code was proposed in 2001 by Daniel Gottesman, Alexei Kitaev, and John Preskill as a way to encode a qubit in an oscillator. The GKP codewords are coherent superpositions of periodically displaced squeezed vacuum states. Because of the challenge of merely preparing the codewords, the GKP code was for a long time considered to be impractical. However, the remarkable developments in quantum hardware and control technology in the last two decades has made the GKP code a frontrunner in the race to build practical, fault-tolerant bosonic quantum technology. In this Perspective, we provide an overview of the GKP code with emphasis on its implementation in the circuit-QED architecture and present our outlook on the challenges and opportunities for scaling it up for hardware-efficient, fault-tolerant quantum error correction.},
	number = {2},
	urldate = {2021-09-17},
	journal = {PRX Quantum},
	author = {Grimsmo, Arne L. and Puri, Shruti},
	month = jun,
	year = {2021},
	note = {Publisher: American Physical Society},
	pages = {020101},
}

@Article{puri2017_ising,
author={Puri, Shruti
and Andersen, Christian Kraglund
and Grimsmo, Arne L.
and Blais, Alexandre},
title={Quantum annealing with all-to-all connected nonlinear oscillators},
journal={Nature Communications},
year={2017},
month={Jun},
day={08},
volume={8},
number={1},
pages={15785},
abstract={Quantum annealing aims at solving combinatorial optimization problems mapped to Ising interactions between quantum spins. Here, with the objective of developing a noise-resilient annealer, we propose a paradigm for quantum annealing with a scalable network of two-photon-driven Kerr-nonlinear resonators. Each resonator encodes an Ising spin in a robust degenerate subspace formed by two coherent states of opposite phases. A fully connected optimization problem is mapped to local fields driving the resonators, which are connected with only local four-body interactions. We describe an adiabatic annealing protocol in this system and analyse its performance in the presence of photon loss. Numerical simulations indicate substantial resilience to this noise channel, leading to a high success probability for quantum annealing. Finally, we propose a realistic circuit QED implementation of this promising platform for implementing a large-scale quantum Ising machine.},
issn={2041-1723},
doi={10.1038/ncomms15785},
url={https://doi.org/10.1038/ncomms15785}
}

@article{wineland2013,
  title={Nobel Lecture: Superposition, entanglement, and raising Schr{\"o}dinger’s cat},
  author={Wineland, David J},
  journal={Reviews of Modern Physics},
  volume={85},
  number={3},
  pages={1103},
  year={2013},
  publisher={APS}
}

@article{kanao_quantum_2022,
	title = {Quantum {Gate} for a {Kerr} {Nonlinear} {Parametric} {Oscillator} {Using} {Effective} {Excited} {States}},
	volume = {18},
	url = {https://link.aps.org/doi/10.1103/PhysRevApplied.18.014019},
	doi = {10.1103/PhysRevApplied.18.014019},
	abstract = {A Kerr nonlinear parametric oscillator (KPO) can stabilize a quantum superposition of two coherent states with opposite phases, which can be used as a qubit. In a universal gate set for quantum computation with KPOs, an Rx gate, which interchanges the two coherent states, is relatively hard to perform owing to the stability of the two states. We propose a method for a high-fidelity Rx gate by exciting the KPO outside the qubit space with parity-selective transitions, which can be implemented by only adding a driving field. In this method, the utilization of higher effective excited states leads to a faster Rx gate, rather than states near the qubit space. The proposed method can realize a continuous Rx gate and thus is expected to be useful for, e.g., recently proposed variational quantum algorithms.},
	number = {1},
	urldate = {2022-09-06},
	journal = {Physical Review Applied},
	author = {Kanao, Taro and Masuda, Shumpei and Kawabata, Shiro and Goto, Hayato},
	month = jul,
	year = {2022},
	note = {Publisher: American Physical Society},
	pages = {014019},
}

@article{paz2020,
  title = {State-dependent motional squeezing of a trapped ion: Proposed method and applications},
  author = {Mart\'{\i}n Drechsler and María Bel\'en Far\'{\i}as and Nahuel Freitas and Christian T. Schmiegelow and Juan Pablo Paz },
  journal = {Phys. Rev. A},
  volume = {101},
  issue = {5},
  pages = {052331},
  numpages = {4},
  year = {2020},
  month = {May},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.101.052331},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.101.052331}
}

@article{Livingston_2022, 
title={Experimental demonstration of continuous quantum error correction}, 
journal = {Nature Communications},
volume={13}, url={http://dx.doi.org/10.1038/s41467-022-29906-0}, DOI={10.1038/s41467-022-29906-0}, abstractNote={<jats:title>Abstract</jats:title><jats:p>The storage and processing of quantum information are susceptible to external noise, resulting in computational errors. A powerful method to suppress these effects is quantum error correction. Typically, quantum error correction is executed in discrete rounds, using entangling gates and projective measurement on ancillary qubits to complete each round of error correction. Here we use direct parity measurements to implement a continuous quantum bit-flip correction code in a resource-efficient manner, eliminating entangling gates, ancillary qubits, and their associated errors. An FPGA controller actively corrects errors as they are detected, achieving an average bit-flip detection efficiency of up to 91%. Furthermore, the protocol increases the relaxation time of the protected logical qubit by a factor of 2.7 over the relaxation times of the bare comprising qubits. Our results showcase resource-efficient stabilizer measurements in a multi-qubit architecture and demonstrate how continuous error correction codes can address challenges in realizing a fault-tolerant system.</jats:p>}, number={1}, journal={Nature Communications}, publisher={Springer Science and Business Media LLC}, 
author={Livingston, William P. and Blok, Machiel S. and Flurin, Emmanuel and Dressel, Justin and Jordan, Andrew N. and Siddiqi, Irfan}, 
journal = {Nature Communications},
volume={13},
year={2022}, month=apr, language={english} }

@article{delsing_new, 
title = {Universal control of a bosonic mode via drive-activated native cubic interactions},
author = {Axel M. Eriksson and Théo Sépulcre and Mikael Kervinen and Timo Hillmann and Marina Kudra and  Simon Dupouy and Yong Lu and Maryam Khanahmadi and Jiaying Yang and Claudia Castillo-Moreno and Per Delsing and Simone Gasparinetti},
journal = {Nature Communications 15, 2512},
year = {2024} }

%, Mikael Kervinen, , Marina Kudra, Simon Dupouy, Yong Lu, Maryam Khanahmadi, Jiaying Yang, Claudia Castillo-Moreno, Per Delsing, Simone Gasparinetti

